Post-quantum Zero Knowledge in Constant Rounds

We construct a constant-round zero-knowledge classical argument for NP secure against quantum attacks. We assume the existence of Quantum Fully-Homomorphic Encryption and other standard primitives, known based on the Learning with Errors Assumption for quantum algorithms. As a corollary, we also obtain a constant-round zero-knowledge quantum argument for QMA. At the heart of our protocol is a new no-cloning non-black-box simulation technique.

==> compiler.tex <==

\section{Round-Preserving Quantum Zero-Knowledge Compiler for Arguments}\label{sec:compiler}
\nir{Not sure what's the role of this section}

In this section we present a round-preserving compiler that compiles any classical-communication argument into a zero-knowledge one.
That is, the compiler compiles a classical-communication argument with $t$ rounds and strong quantum soundness, into a classical-communication argument with $O(t)$ rounds, strong quantum soundness \emph{and} quantum zero-knowledge.
The compiler takes any classical-communication protocol $\prot{\zkP}{\zkV}$ and transforms it into a new protocol $\prot{\compP}{\compV}$.
The compiler has two versions;one that uses weaker computational assumptions but require more communication rounds, and another with (seemingly) stronger computational assumptions and less communication rounds.
We will start with describing the simpler version, which is the second version.\nir{The above text is old? we don't have two version anymore, right?}

\paragraph{Ingredients and notation:}
\begin{itemize}
\item
A $k$-round protocol $\prot{\zkP}{\zkV}$ for $\lang$... \nir{the protocol you start from }

\item
%A non-interactive commitment scheme $( \COM, \VER)$ with statistical binding and computational hiding against $\QPT$ machines. \nir{to be consistent with other defs, call it quantum computational hiding and define it accordingly}
\item
A perfectly correct\nir{remove, just define it to be perfectly correct to begin with}, secret-key encryption scheme $(\ske, \skd)$, secure against $\QPT$ adversaries. \nir{again, "quantum secure" or something of that sort}
\item
A secure function evaluation scheme $(\sfeEnc, \sfeEval, \sfeD)$ with quantum input privacy and statistical circuit privacy.


\nir{Moved the circuit to the protocol, made it simpler.
	For $\secp \in \Nat$, denote by $k(\secp) = k$ the number of rounds in the original protocol $(\zkP, \zkV)$ on an input of length $\secp$, and by $\ell(\secp) = \ell$ the number of random bits used by $\zkV$ on an input of length $\secp$.
	For every $x \in \{0, 1\}^{\secp}, i \in [k], r \in \{0, 1\}^{\ell}$, Denote by $C_{x, i, r}$ the $i$-th message function of $\zkV$ with randomness $r$ on joint input $x$.
	Now, again for $\secp \in \Nat$, denote the set of circuits $\mathcal{C}_{\secp} = \{ C_{x, i, r} \}_{x \in \zo^\secp, i \in [k], r \in \{0, 1\}^{\ell}}$ and $\mathcal{C} =\{\mathcal{C}_{\secp}\}_{\secp \in \Nat}$.
}

\item
A classical zero-knowledge proof system for $\NP$, $(\zkP_{\mathsf{zk}}, \zkV_{\mathsf{zk}})$, with statistical soundness \nir{better write argument and later argue that if we use statistical and underlying system is proof then so is this etc...} and computational zero-knowledge against $\QPT$ machines.

\item
A two-message, function hiding, secure function evaluation scheme, with both sender and receiver privacy against $\QPT$ machines.
\end{itemize}
%
We describe the protocol in \figref{fig:compiled_prot}.











\iffalse
\protocol
{\proref{fig:compiled_prot}}
{The compiled protocol between $\compP$ and $\compV$, based on the original protocol between $\zkP$ and $\zkV$.}
{fig:compiled_prot}
{
	\begin{description}
	\item[Common Input:] An instance $\ins \in \lang\cap \zo^\secp$, for security parameter $\secp \in \Nat$.
	\item[$\compP$'s private input (optional):] A (classical or quantum) witness.
	\end{description}
	
	
	\begin{enumerate}
	\item
	{\bf Commitment Initialization:} $\compP$ samples a secret key $sk\gets \zo^\secp$ for the encryption scheme $\SKE$, and a commitment $c \gets \Com(sk)$. The commitment $c$ is then sent to $\compV$.
	
	\item
	{\bf Protocol Emulation:} The parties emulate an execution of $\prot{\zkP}{\zkV}$ as follows. At the onset of the protocol, they each choose randomness $R_\zkP,R_\zkV$ for $\zkP$ and $\zkV$, respectively.
	
	\smallskip
	For every round $i\in [k]$:
	\begin{itemize}
	\setlength{\itemindent}{-.2in}
	
	\item $\compP$ computes $\zkP$'s $i$-th message $p_i$, an SFE encryption $(\ciph_i,\sk_i) \gets \sfeEnc(p_1, \cdots, p_i)$, and a plain encryption $c_i \gets \ske_{sk}(p_i)$. It sends $(\ciph_i,c_i)$ to $\compV$.
	\omri{I think there was a slight typo there, here is the original: $\compP$ computes $\zkP$'s $i$-th message $p_i$, an SFE encryption $(\ciph_i,\sk_i) \gets \sfeEnc(p_i)$, and a plain encryption $c_i \gets \ske_{sk}(p_1,\dots,p_i)$. It sends $(\ciph_i,c_i)$ to $\compV$.}
	
	\item
	$\compV$ evaluates $\evciph_i \gets \sfeEval(\zkV_{i},\ciph_i)$, where the circuit $\zkV_i$ has input $p_1,\dots,p_i$, and computes the next message $v_i$ of $\zkV$ given common input $x$, randomness $R_\zkV$, and prover messages $p_1,\dots,p_i$. It sends $\evciph_i$ to $\compP$.
	\omri{I slightly changed the original item you wrote, I changed it to make sure it's clear that the input to $\zkV_i$ is only the prover messages so far, the rest (i.e. $x$ and $R_\zkV$) is hardwired into the circuit, right? here is the original item:
		$\compV$ evaluates $\evciph_i \gets \sfeEval(\zkV_{i},\ciph_i)$, where the circuit $\zkV_i$ computes the next message $v_i$ of $\zkV$ given input $x$, randomness $R_\zkV$, and prover messages $p_1,\dots,p_i$. It sends $\evciph_i$ to $\compP$.}
	
	\item
	$\compP$ decrypts $v_i \gets \sfeD_{\sk_i}(\evciph_i)$, and proceeds to the next round of emulation.
	
	\end{itemize}
	
	\item
	{\bf Verifier Consistency:} $\compV$ sends $R_\zkV$ to $\zkP$, who checks that all $\zkV$ messages $v_1,\dots,v_k$ deduced through the protocol are consistent (correspond to an execution of $\prot{\zkP}{\zkV}(x)$ with randomness $R_\zkP$ and $R_\zkV$, respectively).
	
	\item
	{\bf Zero Knowledge Proof:} $\compP$ and $\compV$ engage in a zero knowledge proof $\prot{\zkP_{\mathsf{zk}}}{\zkV_{\mathsf{zk}}}$ where $\compP$ proves consistency. Specifically, $\compP$ provers that there exist messages $p_1,\dots,p_k$, secret key $sk$, and decryption keys $\sk_1,\dots,\sk_k$ such that:
	\begin{itemize}
	\item $c\in \Com(sk)$: $c$ is a commitment to $sk$.
	\item $c_i \in \ske_{sk}(p_i)$: each $c_i$ is an encryption of $p_i$.
	\item $(\ciph_i,\sk_i) \in \sfeEnc(p_1,\dots,p_i)$: each $\ciph_i$ sent in the protocol is an SFE encryption of $p_1,\dots,p_i$ with corresponding decryption key $\sk_i$.
	\item
	One of the following occurs:
	\begin{enumerate}
	\item
	In an execution of the verifier $\zkV$ with input $x$, randomness $R_\zkV$, and prover messages $p_1,\dots,p_k$, $\zkV$ accepts.
	\item
	Let $v_1',\dots,v_k'$ be the verifier messages in the latter execution, then for some $i$, the evaluated ciphertext $\evciph_i$ sent by the verifier is inconsistent: $\sfeD_{\sk_i}(\evciph_i) \neq v_i'$.
	\end{enumerate}
	\end{itemize}
	
	\item
	{\bf Acceptance:}
	$\compV$ accepts if $\zkV_{\mathsf{zk}}$ does.
	
	\end{enumerate}
}
\fi












\subsubsection{Analysis}

\begin{proposition}
The compiled protocol $(\compP, \compV)$ is computational zero-knowledge against quantum machines.
\end{proposition}

\begin{proof}


\end{proof}











We now analyze the protocol. We first show that it is computationally sound against malicious quantum provers, and then that it is $\ZK$ against quantum verifiers.

\begin{proposition}
If the protocol $(\zkP, \zkV)$ is statistically sound, then $(\compP, \compV)$ (that is, \proref{fig:compiled_prot}) is statistically sound.
\end{proposition}
\begin{proposition}
If the protocol $(\zkP, \zkV)$ is computationally sound against quantum provers, then $(\compP, \compV)$ (that is, \proref{fig:compiled_prot}) is computationally sound against quantum provers.
\end{proposition}
\begin{proposition}
If the protocol $(\zkP, \zkV)$ is (classically) computationally sound, then $(\compP, \compV)$ (that is, \proref{fig:compiled_prot}) is (classically) computationally sound.
\end{proposition}
We will prove Proposition 3.2 below. \omri{After writing the proof, check what modifications (if any) are needed to adust it to any of the other two propositions.}

\begin{proof}
Assume toward contradiction that $(\compP, \compV)$ is not quantum computationally sound, that is, there exists a non-uniform $\QPT$ prover $\compmP = \set{ \zkP^{*}_{\mathsf{zk}, \secp} }_{\secp \in \Nat}$ and a noticeable probability function $\varepsilon(\secp) =\secp^{-O(1)}$, s.t. for infinitely many values of $\secp$, there is an instance $\ins \in \{0, 1\}^{\secp}\setminus \lang$ s.t. $\view_{\compV}\prot{\zkP^{*}_{\mathsf{zk}, \secp}}{\compV}(\ins) = 1$ with probability $\varepsilon(\secp)$.

We will describe a successfully cheating n.u. $\QPT$ prover $\zkmP = \{ \zkmP_{\secp} \}_{\secp \in \Nat}$ for the original protocol $(\zkP, \zkV)$.
Fix $\secp\in\Nat$ and $\ins\in \zo^\secp\setminus \lang$ such that $\zkP^{*}_{\mathsf{zk}, \secp}$ convinces $\compV$ of accepting with noticeable probability, we will describe $\zkmP_{\secp}$ (from now on, we will drop the subscript $\secp$, when it is clear from the context).

It is a known fact in cryptography (and more broadly, in computational complexity theory) that non-uniform circuit families can be assumed, without the loss of generality, to be deterministic rather than randomized.
The same cannot be assumed for quantum circuits; general quantum circuits include measurements, and measurements implicitly induce random experiments (namely, the output of the measurement is a random variable), and this in particular is relevant in the setting of interactive quantum algorithms.
However, there is one very specific thing we can assume w.l.o.g. when dealing with quantum n.u. adversaries; If the first message in the protocol is the adversary's, then we can consider it fixed.

More precisely, recall that $\compmP$ is a quantum interactive algorithm, which means that its input is a message and an inner quantum state, and its output is also in the same structure (the output message is sent to the other side, the inner quantum state is not sent and is kept as an input inner state for the next round).
Given that the adversary $\compmP$ needs to send the first message of the protocol, consider the pair $m_{1}, s_{1}$ (message and inner quantum state) that maximizes, over the random coins of $\compV$ and all further quantum measurement outcomes made by $\compmP$, the probability that $\compV$ will accept, and accordingly choose $m_{1}, s_{1}$ to be the (quantum) non-uniform advice that $\compmP$ receives.
Note that in our specific case $m_1$ is a classical message.

A second thing we can assume, is that when $\compmP$ interacts with $\compV$, the $\NP$ statement that $\compmP$ proves to $\compV$ at the end of interaction is true with noticeable probability, and this is due to the binding of the commitment $\Com$, the soundness of $(\zkP_{\mathsf{zk}}, \zkV_{\mathsf{zk}})$, and to the fact that $\compmP$ succeeds w.p. $\secp^{-O(1)}$ to convince $\compV$ and thus in particular succeeds to convince $\zkV_{\mathsf{zk}}$.
In particular, with noticeable probability $\compmP$ indeed commits to a key $sk$ on its first message (and it is always the same key, as we assume w.l.o.g. that the first message is always the same).

We can now describe $\zkmP$.
\begin{enumerate}
\item
Recall that the non-uniform advice of $\zkmP$ is the classical secret key $sk$ along with the first (classical) message and inner quantum state $m_{1}, s_{1}$.
$\zkmP$ takes the part of $m_{1}$ that's $\ske_{sk}(p_{1})$, decrypts it using $sk$ to get $p_{1}$ and sends it to $\zkV$.\footnote{As a technicality, if a message $m_{\compmP}$ is not in the structure of (encryption of (1st string), 4th string), $\zkmP$ just sends $\bot$ to $\zkV$, who rejects immediately.}
\item
For $i = 1, 2, \cdots, k - 1$:
\begin{enumerate}
\item
$\zkV$ returns the message $v_i := \zkV_i(p_{1}, \cdots, p_{i})$.
\item
From the circuit privacy property of the SFE, we have the simulator $\HESim$.
$\zkmP$ executes $\ciph_i' \gets \HESim((p_{1}, \cdots, p_{i}), \zkV_i(p_{1}, \cdots, p_{i}))$, it then takes the previous inner quantum state $s_{i}$ that $\compmP$ outputted, and feeds the input $(\evciph'_i, s_i)$ to $\compmP$.
$\compmP$ outputs a new message and inner quantum state $m_{i + 1}, s_{i + 1}$.

$\zkmP$ takes the part of $m_{i + 1}$ that's $\ske_{sk}(p_{i + 1})$, decrypts it using $sk$ to get $p_{i + 1}$ and sends it to $\zkV$.
\end{enumerate}
\item
$\zkV$ accepts or rejects with accordance to the given transcript and its private randomness.
\end{enumerate}

We saw the protocol, where $\zkmP$ uses $\compmP$ on one side and interacts with $\zkV$ on the other, and we would like to say that the interactions that are generated in both cases are statistically indistinguishable, that is, if we look at the random variable which is the interaction between $\compmP$ and the true compiled verifier $\compV$, and on the random variable which is the interaction between $\compmP$ and what $\zkmP$ simulates for it, these random variables are statistically indistinguishable.

Observe that if we indeed manage to show this statistical indistinguishability, then it is necessarily the case that with noticeable probability, $\zkmP$ convinces $\zkV$ to accept - let us now formalize what we just said.
For every $\secp \in \Nat$, fix $x_\secp \in \zo^\secp \setminus \lang$ and first message that maximizes the chances of the malicious prover $\compmP$ to cheat, and we will define two ensembles of random variables $X_{\HESim} = \{ X_{\HESim, \secp} \}_{\secp \in \Nat}, \; X_{\mathsf{Eval}} = \{ X_{\mathsf{Eval}, \secp} \}_{\secp \in \Nat}$ (like before, from now on the subscript $\secp$ is dropped when the context is clear).

\begin{itemize}
\item $X_{\HESim}$:
Randomness $R_{\zkV}$ for $\zkV$ is chosen, then follows an interaction between $\compmP$ and $\zkmP$, where $\zkmP$ uses $\zkV$ with randomness $R_{\zkV}$ in the communication to compute its messages.
Note that this is just the $\compmP \leftrightarrow \zkmP$ part of the interaction from the above soundness reduction.
There is only one adjustmen to the interaction: At the end of interaction, if at some point of the interaction an inconsistent message was sent from $\compmP$ (i.e. a message that is either unstructured, or does not maintain the consistency requirement from \proref{fig:compiled_prot}) then the output of $X_{\HESim}$ is just $\bot$, otherwise it is all $k$ messages that $\compmP$ sent, and the randomness $R_{\zkV}$ of $\zkV$.

\item $X_{\mathsf{Eval}}$:
Similarly to $X_{\HESim}$, begins with sampling $R_\zkV$, but this time the interaction is between $\compmP$ and the original $\compV$, where $\compV$ uses the randomness $R_\zkV$ for $\zkV$.
Also similarly to before, it is checked at the end that if $\compmP$ sent an inconsistent (or unstructured) message, $\bot$ is the output, and if not, then the output of the random variable is the messages of $\compmP$, and $R_\zkV$.
\end{itemize}
Observe that the main (and only, actually) difference between the two interactions above is that for a given message $(\ske_{sk}(p_{i})\; , \; \ciph_i)$ from $\compmP$, in $X_{\HESim}$, we decrypt the secret-key encryption ciphertext to get $p_{i}$, compute $\zkV_i(p_{1}, \cdots, p_{i})$ and use the simulator $\HESim$ so that we can return to $\compmP$ the message $\HESim((p_{1}, \cdots, p_{i}), \, \zkV_i(p_{1}, \cdots, p_{i}))$, while in $X_{\mathsf{Eval}}$, we just compute $\evciph_i \gets \sfeEval(\zkV_i, \, \ciph_i)$ and return to $\compmP$ the message $\evciph_i$.
We can now state our claims:
\begin{claim}
Assume that $X_{\HESim} \approx_s X_{\mathsf{Eval}}$, then for infinitely many values of $\secp$, the interaction between $\zkmP_{\secp}$ and $\zkV_\secp$ on common input $x_\secp$ yields a successful verification with noticeable probability.
\end{claim}
\begin{proof}
First, recall we know that when $\compmP$ interacts with $\compV$, there is a noticeable probability that $\compV$ accepts.
It is thus follows from this fact, and from the fact that $\Com$ is binding, the SFE has perfect correctness, and from the soundness of the protocol $(\zkP_{\mathsf{zk}}, \zkV_{\mathsf{zk}})$, that there is a noticeable probability that the hidden transcript inside the encryptions that $\compmP$ sends is both consistent and accepting.
It follows that if we get a transcript from $X_{\mathsf{Eval}}$, there's a noticeable probability that we don't get $\bot$, and not only that, but that if we take the messages that $\compmP$ sent, decrypt them to get for every $i \in [k]$ the message $p_{i}$, feed $(p_{1}, \cdots, p_{k})$ to the verification circuit of $\zkV$ with randomness $R_\zkV$, we get $\zkV_k(p_{1}, \cdots, p_{k}) = 1$.

On the other hand, assume towards contradiction that when $\compmP$ interacts with $\zkV$ through $\zkmP$, then $\zkV$ accepts only with negligible probability.
This implies in particular, that when we get the transcript from $X_{\HESim}$ there's a negligible probability that $\zkV_k(p_{1}, \cdots, p_{k}) = 1$ (and of course, that the output is not $\bot$).
Because $R_\zkV$ is part of the view in both of the random variables, it can be seen that by this procedure we can distinguish between the two random variables.

More precisely, We can construct a distinguisher that gets an unknown $X$ (either $X_{\mathsf{Eval}}$ or $X_{\HESim}$), takes the messages after decryption $(p_{1}, \cdots, p_{k})$, the randomness $R_\zkV$, computes $\zkV_k(p_{1}, \cdots, p_{k})$ and outputs whatever the verification circuit outputs (if the output was $\bot$, the distinguisher outputs 0).
We deduce that on $X_{\mathsf{Eval}}$ the distinguisher outputs 1 with noticeable probability, but on $X_{\HESim}$ only with negligible probability, and thus distinguishes with noticeable advantage the two random variables, in contradiction to $X_{\mathsf{Eval}} \approx_s X_{\HESim}$.
\end{proof}

With accordance to the above, all that's left to prove in order to finish the soundness proof is that indeed $X_{\HESim} \approx_s X_{\mathsf{Eval}}$.
\begin{claim}
$$
X_{\HESim} \approx_s X_{\mathsf{Eval}} \enspace .
$$
\end{claim}
\begin{proof}
To prove the above statistical indistinguishability we will use a standard hybrid argument and an averaging argument, plus the statistical circuit privacy of the SFE.
Assume towards contradiction that there is a n.u. (unbounded) distinguisher $\Disting = \{\Disting_\secp\}_{\secp \in \Nat}$ that distinguishes with noticeable advantage between the two distributions.
Consider the following $k$ hybrid distributions: for $i \in \{0, 1, \cdots, k - 1 \}$, define $H_i$ to be the random variable that describes an interaction, s.t. until and including message $i$, the returned messages to $\compmP$ are according to the same rules as in $X_{\mathsf{Eval}}$, and from message $i + 1$, according to the rules of $X_{\HESim}$, and deduce that $H_0 = X_{\HESim}$, $H_{k - 1} = X_{\mathsf{Eval}}$.
By triangle inequality of statistical distance, there is some $i \in \{ 0, 1, \cdots, k - 2 \}$ s.t. $\Disting$ can distinguish with noticeable probability between $H_i$ and $H_{i + 1}$.

We will now need to get into some technical details and we'll begin with breaking down the processes of generating a sample from $H_{i}$ or $H_{i + 1}$ into parts.
So, how is a sample from $H_{i + b}$ is generated? The first part of the two is the same; $\compmP$ outputs the first message and state $(m_{1}, s_{1})$, then we take $\ciph_1$ out of $m_{1}$ and compute $\evciph_1 \gets \sfeEval(\zkV_1, \ciph_1)$.
$\compmP$ takes $\evciph_1$ to compute its next output $(m_{2}, s_{2})$, and so on until and including the $(i + 1)$-th output $(m_{i + 1}, s_{i + 1})$ of $\compmP$.
Let's call the random variable that denotes the output of this process (which is a subprocess inside the process of generating a sample for either $H_{i}$ or $H_{i + 1}$) with $Y$, that is, the output of $Y$ is the randomness $R_\zkV$, the messages $(m_{1}, \cdots, m_{i + 1})$ of $\compmP$ and the latest quantum inner state $s_{i + 1}$.\footnote{
	Note that the random variable $Y$ is a quantum random variable, that is, an r.v. that part of its output is a register of qubits.
	Two different ways to treat this formally in our current setting is to either assume w.l.o.g. that $\mathcal{D}$ have quantum capabilities as it is unbounded, or to just define the $s_{\compmP, i + 1}$ part of $Y$'s output to be the (exponentially large) classical unit vector representation of the quantum state $s_{\compmP, i + 1}$, and thus make $Y$ a classical random variable.}

After generating a sample from $Y$, the procedures of generating a sample from $H_{i}$ or $H_{i + 1}$ diverge.
\begin{itemize}
\item
In $H_{i}$, we decrypt all previous messages to get $p_1, \cdots, p_{i + 1}$, compute $v_{i + 1} := \zkV_{i + 1}(p_{1}, \cdots, p_{i + 1})$, and return to $\compmP$ the simulation of the evaluated ciphertext
$$
\ciph_{i + 1}'\gets \HESim((p_{1}, \cdots, p_{i + 1}), \zkV_{i + 1}(p_{1}, \cdots, p_{i + 1})) \enspace .
$$
\item
In $H_{i + 1}$, for the message $m_{i + 1} = (\ske_{sk}(p_{i + 1}) \; , \; \ciph_{i + 1})$, we just return the evaluated ciphertext $\evciph_{i + 1} \gets \sfeEval(\zkV_{i + 1}, \ciph_{i + 1})$.
\end{itemize}
In both cases above, after the $(i + 1)$-th response sent to $\compmP$, all returned messages to $\compmP$ are generated by the same rules as in $X_{\HESim}$, that is, we just return simulations of evaluated ciphertexts.

By an averaging argument, the above implies that there is a sample
$$
y := (R_\zkV', (m'_{1}, \cdots, m'_{i + 1}), s'_{i + 1})
$$
in the image of $Y$ that maximizes the distinguishability of $\Disting$ between the two cases.
Observe that the messages $(m'_{1}, \cdots, m'_{i + 1})$ necessarily maintain structure and consistency, because if we assume towards contradiction that they do not, considering the fact that $y$ is a distinguishability-maximizing prefix of the interaction, and the fact that for an interaction where there's an inconsistent (or unstructured) message, the output of the r.v. is always $\bot$, we get $\Delta_{\Disting}(H_i, H_{i + 1}) = 0$.

It is left to see that we can use $y$ to break the circuit privacy of the SFE: consider the circuit $\zkV_{i + 1}$ (which is the circuit that for input $p_1, \cdots, p_{i + 1}$, outputs the output of $\zkV$ when the common input is $x$ and its randomness is $R_\zkV'$), an input for the circuit $(p'_{1}, \cdots, p'_{i + 1})$ and a legal ciphertext $\ciph_{i + 1}$.
We can distinguish (with noticeable probability) between just evaluations of the circuit on the input, and simulations of evaluations.

This distinguishing can be done by getting an evaluation (or simulated evaluation) ciphertext $\ciph'_{i + 1}$, using $y$ to continue the interaction, and sending the final interaction to $\Disting$.
If the $\ciph'_{i + 1}$ was a simulated evaluation then the interaction is a continuation of $y$ to a sample from $H_{i}$, and if $\ciph'_{i + 1}$ was a true evaluation then the interaction is a continuation of $y$ to a sample from $H_{i + 1}$.
\end{proof}

This concludes our proof of soundness.
\end{proof}

\omri{A few comments about the modifications to the above proof, s.t. it will hold as a proof for propositions 3.1 and 3.3 respectively.}
















\begin{proposition}\label{prp:sim}
\proref{fig:wzk_prot} is weak zero-knowledge against explainable verifiers.
\end{proposition}

\begin{proof}
\def \ranmal {r^*}
We describe the simulator $\zkS$. Throughout, we assume w.l.o.g that the malicious verifier $\zkmV$ outputs its view consisting of its random coins and prover messages.
(Otherwise, we consider a new verifier of this form, along with a new distinguisher who computes internally the original verifier output, and then applies the original distinguisher.)

\medskip
\paragraph{$\zkS(\ins,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon})$:}
\begin{enumerate}
\item
Sample coins $\ranmal$ for $\zkmV_\secp$. Henceforth, $\zkmV_{\ranmal}$ denotes the corresponding (deterministic) verifier.
\item
Sample a random $r'\gets \zo^\secp$ and a first commitment message and state $(\cm_1,\tau)\gets \comS(r')$ corresponding to a commitment to $r'$. Store the randomness $r_{\cm}$ used to generate the commitment. Feed $\cm_1$  to $\zkmV_{\ranmal}$.
\item
If the verifier aborts, output $(\ranmal,\cm_1,\bot)$.
\item \label{stp:ver_mes}
Obtain $(\cm_2,\cmt,\zkVCT,\obfC, \zkVCT',\rsrePK',\wi_1)$ from $\zkmV_{\ranmal}$
\item
Compute the third commitment message $\cm_3 \gets \comS(\cm_1,\cm_2;\tau)$.
\item
Construct the ({\em homomorphic simulation}) circuit $\HC(r)$ that given an input $r$:
\begin{itemize}
\item
Construct a distinguisher $\rsremD'(\zkPCT)$ for the RSR encryption that given a ciphertext $\zkPCT$:
\begin{itemize}
\item
Samples at random a second $\WI$ message $$\wi_2 \gets \wiP(\Psi,r,\wi_1)$$
for the statement $\Psi(\ins,\cmt,\obfC,\zkPCT,\rsrePK',\cm_1,\cm_2,\cm_3)$, using as the witness the randomness $r$ attesting that $\cmt=\Com(0;r)$.
\item
Runs $\zkmD_\secp(\ranmal,\cm_1,(\cm_3,\zkPCT,\wi_2))$.
\end{itemize}
\item
Applies the decryptor
$$
\tilde u \gets \rsretD^{\rsremD'}(\zkVCT',\rsrePK',1^{1/\varepsilon})\enspace,
$$
and output $\tilde u$.
\end{itemize}
All randomness required by the above is hardwired into $\HC$.
\item
Compute $\evciph = \fheEv(\HC,\zkVCT)$.

\item \label{stp:td1}
If $\obfC(\evciph)=1$:
\begin{itemize}
\item
Sample $\zkPCT\gets \rsreE_{\rsrePK'}(1)$.
\item
Sample a second $\WI$ message
$$\wi_2 \gets \wiP(\Psi,\evciph,\wi_1)$$
for the statement $\Psi(\ins,\cmt,\obfC,\zkPCT,\rsrePK',\cm_1,\cm_2,\cm_3)$, using as the witness $\evciph$ attesting that $\obfC(\evciph)=1$.
\end{itemize}
\item
Otherwise:\label{stp:td2}
\begin{itemize}
\item
Compute $\zkPCT =  \rsreE_{\rsrePK'}(0;r')$, where $r'$ is the randomness underlying the extractable commitment.
\item
Sample a second $\WI$ message
$$\wi_2 \gets \wiP(\Psi,(r',r_\cm),\wi_1)$$
for the statement $\Psi(\ins,\cmt,\obfC,\zkPCT,\rsrePK',\cm_1,\cm_2,\cm_3)$, using as the witness the randomness $r'$ attesting that $\zkPCT\gets \rsreE_{\rsrePK'}(0;r')$ and the commitment randomness $r_\cm$.
\end{itemize}
\item
Output $(\ranmal,\cm_1,(\cm_3,\zkPCT,\wi_2))$.
\end{enumerate}

\paragraph{Simulation validity.} The simulator clearly runs in polynomial time (in its input length). We focus on proving validity. Let $\zkmV=\set{\zkmV_\secp}_\secp$ be a polynomial-size explainable verifier, let $\zkmD=\set{\zkmD_\secp}_\secp$  be a polynomial-size distinguisher, and let $\varepsilon(\secp)=\secp^{-O(1)}$.
% Fix any $\secp$, and $x\in \lang\cap\zo^\secp$ such that the message sent by $\zkmV_\secp$ is explainable (i.e., it is consistent with some honest verifier message as specified in \proref{fig:wzk_prot}).

We consider a sequence of hybrid simulators that transition from the simulator to the prover, and prove that the views generated by each two consecutive hybrids are indistinguishable.

\paragraph{$\zkS_0$:} This is the real simulator $\zkS$.

\paragraph{$\zkS_1$:} This simulator is the same as $\zkS$, only that in Step \ref{stp:td2}, if it needs to give an argument (due to unsuccessful extraction of a proper $\evciph$), it uses the witness $\wit$, instead of $(r',r_\cm)$.


\paragraph{$\zkS_2$:} This simulator is the same as $\zkS_1$, only that instead of an extractable commitment $(\cm_1,\cm_2,\cm_3)$ to $r'$, it provides a commitment to $0^\secp$.

\paragraph{$\zkS_3$:} This simulator is inefficient. It acts the same as $\zkS_2$, only that:
\begin{itemize}
\item
It checks whether, the verifier's message is explainable; namely, in the support of the honest verifier messages (or $\bot)$, and aborts if its not.
\item
Then it finds the commitment randomness $r$, and uses it to provide proofs both in Step \ref{stp:td1} and in Step \ref{stp:td2}.
\end{itemize}

\paragraph{$\zkP_1$:} This simulator is also inefficient. It acts the same as the honest prover $\zkP$, only that:
\begin{itemize}
\item
It checks whether, the verifier's message is explainable; namely, in the support of the honest verifier messages (or $\bot)$, and aborts if its not.
\item
Then it finds the commitment randomness $r$, and uses it to provide the \WI argument.
\end{itemize}

\paragraph{$\zkP_0$:} This simulator emulates the real prover.

To deduce the validity of the simulator, we prove:
\begin{claim}\label{clm:wzk_main}
There exists a negligible $\nu(\secp)$ such that for all $\secp\in\Nat$, $\ins\in\lang\cap\zo^\secp$, $\wit\in\RL(\ins)$, $i\in [3]$,
\begin{align*}
\zkS_{i-1}(\ins,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon})
&\approx_{\zkmD_\secp,\nu}
\zkS_{i}(\ins,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon})\enspace,\\
\zkS_{3}(\ins,\zkmV_\secp,\zkmD_\secp,1^{1/\varepsilon})
&\approx_{\zkmD_\secp,\varepsilon+2^{-\secp}}
\view_{\zkmV_\secp}\prot{\zkP_1(\wit)}{\zkmV_\secp}(\ins) \enspace,\\
\view_{\zkmV_\secp}\prot{\zkP_1(\wit)}{\zkmV_\secp}(\ins)  &\approx_{\zkmD_\secp,\nu}
\view_{\zkmV_\secp}\prot{\zkP(\wit)}{\zkmV_\secp}(\ins)\enspace.
\end{align*}
\end{claim}

\begin{proof}
We prove the indistinguishability of each two consecutive hybrid simulators.

\medskip\noindent
\underline{$\zkS \approx \zkS_1$:} Recall that the only difference between these two simulators is that $\zkS_1$ uses the witness $\wit$ in Step \ref{stp:td2}, instead of $(r',r_{\cm})$. Assume toward contradiction that $\zkmD$ distinguishes the views generated by the two simulators with noticeable probability $\delta(\secp)$. We use $\zkmD$ to construct a verifier $\wimV$ that breaks witness indistinguishability of the underlying $\WI$ argument.

$\wimV$ runs $\zkS$ to sample a transcript, but discards the $\WI$ argument $\wi_2$ that $\zkS$ produces. Instead, it outputs as the first \WI message the message $\wi_1$ produced by $\zkmV$ during the simulation, as well as the statement $\Psi$ and $\wit_0=(r',r_\cm)$ and $\wit_1 = \wit$ as the two witnesses. It then receives a \WI second message $\wi_2'$ generated using one of these witnesses $\wit_i$. It then runs $\zkmD$ on the corresponding view $(\ranmal,\cm_1,(\cm_3,\zkPCT',\wi_2')$, which is identical to that generated by $\zkS$, except that $\wi_2$ generated by $\zkS$ is replaced by the $\wi_2'$ received from the challenger. $\wimV$ outputs whatever $\zkmD$ outputs.

It is left to observe that for each $i\in\zo$, the generated view is distributed identically to that generated by $\zkS_i$. It follows that $\wimV$ has advantage $\delta$ in the \WI challenge.

\medskip\noindent
\underline{$\zkS_1 \approx \zkS_2$:} Recall that the only difference between these two simulators is that $\zkS_2$ commits to $0^\secp$ instead of to $r'$ like $\zkS_1$. Assume toward contradiction that $\zkmD$ distinguishes the views generated by the two simulators with noticeable probability $\delta(\secp)$, then we construct a receiver $\commR$ that breaks the indistinguishability of the extractable commitment with the same advantage $\delta$.

$\commR$ emulates $\zkS_1$, when sampling $r'$, $\commR$ submits to the challenger $s_1=r'$ and $s_2 = 0^\secp$. Then, instead of sampling $\cm_1$ as part of the simulation, $\commR$ obtains it from an outside challenger. It proceeds with the emulation of $\zkS_1$, feeding $\cm_1$ to $\zkmV$, and obtaining $\cm_2$ as part of $\zkmV$'s message. $\commR$ sends  $\cm_2$ to the challenger and obtains $\cm_3$. It hen performs the rest of the emulation using $\cm_3$ (note that $\zkS_1$ no longer requires the randomness underlying the commitment in Step \ref{stp:td2}).

It is left to observe that for each $i\in\set{1,2}$, when the challenger commits to $s_i$, the generated view is distributed identically to that generated by $\zkS_i$. It follows that $\commR$ has advantage $\delta$ in the \WI challenge.

\medskip\noindent
\underline{$\zkS_2 \approx \zkS_3$:} Recall that the difference between these two simulators is that $\zkS_3$ aborts if the verifier's message is not explainable, and if it is uses the commitment randomness $r$ as the witness in Steps \ref{stp:td1} and $\ref{stp:td2}$, instead of $\evciph$ and $\wit$, respectively. Assume toward contradiction that $\zkmD$ distinguishes the views generated by the two simulators with noticeable probability $\delta(\secp)$. We use $\zkmD$ to construct a verifier $\wimV$ that breaks witness indistinguishability of the underlying $\WI$ argument. While the simulator $\zkS_3$ is inefficient, $\wimV$ will be efficient (albeit non-uniform).

First note that the first messages $\cm_1$ of the two simulators are distributed identically. Furthermore, since $\zkmV$ is explainable, there exists a negligible $\mu(\secp)$ such that except with probability $\mu$ over the choice of first message and randomness $\ranmal$ for $\zkmV_\secp$, the verifier's message is explainable. Thus by averaging there exists a fixed first message $\cm_1$ and randomness $\ranmal$ such that conditioned on $(\cm_1,\ranmal)$, $\zkmD_\secp$ distinguishes $\zkS$ from $\zkS_1$ with advantage $\delta-\mu$ and the verifier's message is explainable. We fix such $(\cm_1,\ranmal)$ non-uniformly, which also fixes the randomness $r$, underlying the verifier's $\zkmV$ commitment (we can assume w.l.o.g that the verifiers message is not $\bot$, because then both simulators abort).

The verifier $\wimV$ has $(\cm_1,\ranmal,r)$ hardwired, as well as the state $\tau$ corresponding to $\cm_1$. It emulates $\zkS_2$ starting from the point it obtains the message from $\zkmV$ (Step \ref{stp:ver_mes}), obtains a corresponding transcript, but discards the $\WI$ argument $\wi_2$ that $\zkS_2$ produces. Instead:
\begin{itemize}
\item If the transcript reaches Step \ref{stp:td1} (corresponding to successful extraction of $\evciph$), $\wimV$ sends the challenger the first $\WI$ message $\wi_1$ generated by $\zkmV$ along with the statement $\Psi$ and witnesses $\wit_2 = \evciph$ and $\wit_3 = r$.
\item
If the transcript reaches Step \ref{stp:td2} (corresponding to unsuccessful extraction of $\evciph$), $\wimV$ sends to the challenger $\wi_1$ and $\Psi$ with witnesses $\wit_2 = \wit$ and $\wit_3 = r$.
\end{itemize}
It then receives a \WI second message $\wi_2'$ generated using one of these witnesses $\wit_i$. It then runs $\zkmD$ on the corresponding view $(\ranmal,\cm_1,(\cm_3,\zkPCT',\wi_2')$, which is identical to that generate by $\zkS_2$, except that $\wi_2$ generated by $\zkS_2$ is replaced by the $\wi_2'$ received from the challenger. $\wimV$ outputs whatever $\zkmD$ outputs.

It is left to observe that for each $i\in\set{2,3}$, the generated view is distributed identically to that generated by $\zkS_i$. It follows that $\wimV$ has advantage $\delta-\mu$ in the \WI challenge.

\medskip\noindent
\underline{$\zkP_1 \approx \zkP$:} We jump to prove this indistinguishability as it is very similar to the previous one (the tired reader is advised to skip it).

Recall that the difference between these two provers is that $\zkP_1$ aborts if the verifier's message is not explainable, and if it is, uses the commitment randomness $r$ as the witness when proving $\Psi$ instead of $\wit$ like $\zkP$. Assume toward contradiction that $\zkmD$ distinguishes the views generated by the two provers with noticeable probability $\delta(\secp)$. We use $\zkmD$ to construct a verifier $\wimV$ that breaks witness indistinguishability of the underlying $\WI$ argument. While the prover $\zkP_1$ is inefficient, $\wimV$ will be efficient (albeit non-uniform).

First note that the first messages $\cm_1$ of the two provers are distributed identically. Furthermore, since $\zkmV$ is explainable, there exists a negligible $\mu(\secp)$ such that except with probability $\mu$ over the choice of first message and randomness $\ranmal$ for $\zkmV_\secp$, the verifier's message is explainable. Thus by averaging there exists a fixed first message $\cm_1$ and randomness $\ranmal$ such that conditioned on $(\cm_1,\ranmal)$, $\zkmD_\secp$ distinguishes $\zkP$ from $\zkP_1$ with advantage $\delta-\mu$ and the verifier's message is explainable. We fix such $(\cm_1,\ranmal)$ non-uniformly, which also fixes the randomness $r$, underlying the verifier's $\zkmV$ commitment (we can assume w.l.o.g that the verifiers message is not $\bot$, because then both simulators abort).

The verifier $\wimV$ has $(\cm_1,\ranmal,r)$ hardwired, as well as the state $\tau$ corresponding to $\cm_1$. It emulates $\zkP$ starting from the point it obtains the message from $\zkmV$ (the third protocol message), obtains a corresponding transcript, but discards the $\WI$ argument $\wi_2$ that $\zkP_1$ produces. Instead, it sends the challenger the first $\WI$ message $\wi_1$ generated by $\zkmV$ along with the statement $\Psi$ and witnesses $\wit_0 = \wit$ and $\wit_1 = r$. It then receives a \WI second message $\wi_2'$ generated using one of these witnesses $\wit_i$. It then runs $\zkmD$ on the corresponding view $(\ranmal,\cm_1,(\cm_3,\zkPCT',\wi_2')$, which is identical to that generate by $\zkP$, except that $\wi_2$ generated by $\zkS_2$ is replaced by the $\wi_2'$ received from the challenger. $\wimV$ outputs whatever $\zkmD$ outputs.

It is left to observe that for each $i\in\set{0,1}$, the generated view is distributed identically to that generated by $\zkP_i$. It follows that $\wimV$ has advantage $\delta-\mu$ in the \WI challenge.

\medskip\noindent
\underline{$\zkS_3 \approx \zkP_1$:} Note that up to receiving the verifier's $\zkmV$ message, and adding the generation of $\cm_3$, the views generated by the two simulators are distributed identically. Thus, to prove $(\zkmD_\secp,\varepsilon+2^{-\secp})$-indistinguishability of these two simulators, it suffices to prove $(\zkmD_\secp,\varepsilon+2^{-\secp})$-indistinguishability conditioned on any fixing of the first prover message, verifier randomness $\ranmal$ and message, and $\cm_3$. Note that if the verifier's message is not explainable, both simulators abort, and thus we concentrate on the case that the verifier's message is explainable. From hereon consider such a fixing and let $r$ be the corresponding randomness.

Let $\Delta$ be the advantage of the probabilistic distinguisher $\rsremD'$ (as defined in the simulation procedure) in distinguishing zero-encryptions from one-encryptions:
\begin{align*}\Delta := \abs{\underset{\rsremD',\rsreE}{\EE}\left[\rsremD'(\rsreE_{\rsrePK'}(0))- \rsremD'(\rsreE_{\rsrePK'}(1))\right]}\enspace.
\end{align*}
%
We consider two cases.

\paragraph{Case 1: $\Delta > \varepsilon$.} Let $u$ be the target string underlying the obfuscated CC program $\obfC$, and recall that $\zkVCT'\in \rsreE_{\rsrePK'}(u)$, due to explainability. Then by the random self reducibility of $\rsre$, with overwhelming probability $1-2^{-\secp}$, over the coins of $\rsretD$, it holds that
$$
\rsretD^{\rsremD'}(\zkVCT',\rsrePK',1^{1/\varepsilon}) = u\enspace,
$$
in which case, $\HC(r) = u$. Assume that this is indeed the case.

By the correctness of $\fhe$, the ciphertext $\evciph=\fheEv(\HC,\evciph)$ obtained by the simulator $\zkS_3$ satisfies:
$$
\fheD_{\fheK}(\evciph) = u\enspace,
$$
and thus by the one-sided correctness of the CC obfuscator $\O$,
$$
\obfC(\evciph) = 1\enspace.
$$
This corresponds to successful extraction of $\evciph$, and will result in the simulator $\zkS_3$ behaving identically to the prover $\zkP_1$ (in Step \ref{stp:td1}) --- sampling $\zkPCT$ as a one encryption and $\wi_2$ using the witness $r$.

Thus, in case 1, we have $(\zkmD_\secp,2^{-\secp})$-indistinguishability.

\paragraph{Case 2: $\Delta \leq \varepsilon$.} Here we consider two sub-cases according to whether the simulator still obtains a ciphertext $\evciph$ such that $\obfC(\evciph)=1$ or not. In case it does obtain such $\evciph$, the simulator behaves exactly like $\zkP_1$. Henceforth, we assume that the simulator does not obtain such a witness, in which case it reaches Step \ref{stp:td2}. Here the difference between the simulator $\zkS_3$ and prover $\zkP_1$ is that the first samples $\zkPCT \gets \rsreE_{\rsrePK'}(0)$, whereas the second samples $\zkPCT \gets \rsreE_{\rsrePK'}(1)$. The advantage of $\zkmD_\secp$ in distinguishing the two is exactly the advantage $\Delta \leq \varepsilon$ of $\rsremD'$. This completes the proof of this case, and of \clmref{clm:wzk_main}.
\end{proof}
\end{proof}


\omri{Insert here comments about the round-heavy version of the compiler, specifically, the assumptions, the construction and the modified analysis.
	Question to take care of: if we use MANY-ROUND SFE, how does the prover proves consistency at the end? that is, formally, what is the exact statement that it proves?} 

==> restricted_quantum_extractable_commitments.tex <==


\omri{This is a cancelled section. I am using it to hold the 1st version of the technical overview.}


%who noticed that due to the nature of quantum information, the main existing technique (and actually, all existing techniques at the time) for proving that a protocol is zero-knowledge, called rewinding, does not work in order to show zero-knowledge against quantum verifiers.
%Over the next few years, some progress was done in the field of QZK protocols and zero-knowledge notions in the quantum setting were investigated \cite{watrous2002limits} \omri{First paper to define quantum statistical ZK}.
%In particular, less strict quantum security notions then zero-knowledge \cite{damgaard2004zero} \omri{They showed security against quantum attacks in the CRS model} were shown, but little progress was seen on the problem of zero knowledge secure against quantum attacks.
%
%The first result \cite{watrous2009zero} that showed a postquantum zero-knowledge protocol exist (for NP), opened the gates for numerous open questions in postquantum security of protocols and since then, we have seen progress in understanding quantum protocols and security, a few examples are below.
%
%%The first result \cite{watrous2009zero} that showed a postquantum zero-knowledge protocol exist (for NP), opened the gates for numerous open questions in postquantum security of protocols and since then, we have seen progress in understanding quantum protocols and security:
%%Unruh \cite{unruh2012quantum} constructs (many-rounds) Proof systems for NP,
%%
%%The first result \cite{watrous2009zero} that showed a postquantum zero-knowledge protocol exist (for NP), opened the gates for numerous open questions in postquantum security of protocols and since then, we have seen progress in understanding quantum protocols and security:
%%Unruh \cite{unruh2012quantum} constructs (many-rounds) Proof systems for NP,
%
%Unruh \cite{unruh2012quantum} shows the existence of proof systems for NP with some knowledge extraction guarantee for restricted quantum provers, based on injective one-way functions.
%Lunemann and Nielsen \cite{lunemann2011fully} and Hallgren, Smith, and Song \cite{hallgren2011classical} developed for the first time zero-knowledge arguments of knowledge (that is, extraction guarantee is for \emph{arbitrary} efficient quantum provers) given the QLWE assumption.
%These two works also were also the first to raise the open question of quantum-secure cryptographic protocols with \emph{constant rounds}, referring specifically to zero-knowledge protocols (either arguments or proofs).
%
%Still witnessing the large gap between the number of classically-secure protocols compared to quantumly-secure ones, in a result \cite{ambainis2014quantum} investigating general postquantum security of classical protocols, Ambainis, Rosmanis and Unruh show that numerous popular classically-secure cryptographic protocols are in fact insecure against quantum attacks, under some computational assumptions, meaning that it was not only the lack of techniques to show quantum security, there is simply a gap between classical and quantum security.
%
%In parallel to quantum-secure protocols for NP, developments on quantum protocols (where both prover and verfier are quantum algorithms) increased, and in particular, strides were made towards constructing zero knowledge protocols for \QMA.
%In a breakthrough result \cite{broadbent2016zero} by Broadbent, Ji, Song and Watrous after a line of works on the problem \cite{ben2006secure, dupuis2010secure, dupuis2012actively, liu2006consistency, morimae2015quantum}, it was shown for the first time that zero knowledge quantum proof systems for \QMA exist, rather then only for \NP.
%In that work, the open question of constant-round zero-knowledge protocols for NP (and also QMA) was raised again.
%
%Finally, regarding zero knowledge protocols (even quantum ones) with quantum security {\bf and} constant rounds, results are much more sparse then in the more general postquantum setting....
%\cite{unruh2016computationally, unruh2016collapse}.
%




%
%\subsection{Introduction to Quantum Zero-Knowledge}\label{subsection:intro_to_qzk}
%We start the technical overview (assuming basic background in classical zero-knowledge protocols) with introducing some concepts and existing solutions from the realm of quantum zero-knowledge (QZK), that is, zero-knowledge protocols that are secure against attacks from polynomial-time quantum algorithms.
%
%Let us first recall how to prove that a protocol is zero-knowledge against classical adversaries, and then see how the main proof technique fails against quantum ones.
%Consider the simplest example \cite{goldreich1986prove} of a classical proof system for \NP that is zero-knowledge against classical attacks; the proof is for the NP-complete language of 3-colorability, the joint input of the protocol is a 3-colorable undirected graph $G = (U, E)$ and the prover's witness input is a legal 3-coloring $c:U \rightarrow [3]$ of the graph's vertices.
%The core construction has constant rounds and constant soundness error, and is presented below.
%
%\paragraph{Protocol $\prot{P(c)}{V}(U,E)$:}\label{intro:protocol}
%\begin{enumerate}
%	\item
%	$P$ chooses a random permutation $\varphi:[3]\rightarrow [3]$, and sends $V$ commitments to all colors after applying the permutation:
%	$$
%	(\Com(\varphi(c(v))) \;|\; v\in U) \enspace.
%	$$
%	\item
%	$V$ samples $e\gets E$ at random and sends $e=(u,v)$ to $P$.
%	\item
%	$P$ opens the commitments corresponding to $u$ and $v$.
%	\item
%	$V$ verifies that the two opened colors are distinct.
%\end{enumerate}
%
%\noindent
%The proof that the above protocol is zero-knowledge is by constructing an expected polynomial-time simulator $S$ that for every (possibly malicious) classical verifier $V^*$, operates as follows to sample an interaction transcript that is computationally indistinguishable from the real interaction with the prover.
%In a nutshell, the simulator's strategy will be to guess $e$, the verifier's challenge, and prepare the "prover's" commitments so that they can convince the verifier to accept, given that the verifier's challenge was indeed $e$, and if the guess was wrong, then the simulator restarts.
%
%\paragraph{Simulation $S(V^*)$:}\label{intro:simulator}
%\begin{enumerate}
%	\item $S$ samples $e'\gets E$ and commitments
%	$$
%	(\Com(0) \;|\; v\in U\setminus e') \enspace.
%	$$
%	For the vertices $v',u'$ of $e'$ it samples $c(v')$ and $c(u')$ to be two distinct random colors in $[3]$.
%	
%	$S$ then emulates $V^*$, sending the simulated commitments.
%	
%	\item $S$ receives $e$ from $V^*$ and:
%	\begin{itemize}
%		\item If $e=e'$, opens the corresponding commitments and concludes the simulation.
%		\item Else, returns to the beginning and performs the entire simulation again.
%	\end{itemize}
%\end{enumerate}
%
%\noindent
%Now, it is easy to see that the above simulator can in fact also work for quantum verifiers, it just needs to be quantum in order to execute the verifier's algorithm.
%The problem arises when we want to get an actual sound proof system and reduce the soundness error of this protocol, which is currently $1 - \frac{1}{|E|}$, to be negligible.
%A sound system is achieved by a simple sequential repetition of the protocol $\poly(|E|)$ times (parallel repetition does not preserve zero-knowledge even in the classical setting, which is a subject by itself).
%In the original protocol the simulator guessed in advance the challenge of the verifier, and the running time of the simulator is efficient because the challenge space is restricted to polynomial size (in our case, it's exactly $|E|$), but in the sound version of the protocol the challenge space size is exponential ($|E|^{\poly(|E|)}$) and the simulator cannot guess in advance - this problem is solved by a technique known in the literature as \emph{rewinding}.
%
%The simulator $\tilde{S}$ for the sound protocol will basically run the simulator $S$ for each of the $\poly(|E|)$ iterations of the core protocol, with one adding: at the end of each successful execution of $S$, $\tilde{S}$ takes a snapshot (i.e. copies and keeps on the side) of the verifier's classical inner state (which can be captured by polynomial-size classical string), so that if $S$ fails in the following iteration and needs to try again to guess which edge the verifier wanted the "prover" to open, it can go back to the beginning of the \emph{current} iteration, and not go back all the way to the beginning of the first iteration.
%
%This ability to copy the verifier's inner state is crucial for the simulation to run in expected polynomial time, and it can now be seen where the technique of rewinding fails to work for quantum circuits: We have a combination of two basic concepts from quantum information theory:
%\begin{itemize}
%	\item General quantum circuits, specifically with measurements, are not reversible transformations, and thus when the simulator uses a quantum verifier's circuit and inner quantum state to compute the verifier's next message (which includes the wanted edge to open), if the simulator fails, the inner state of the verifier is lost and cannot be reconstructed.
%	
%	\item General unknown quantum states cannot be copied, and thus the simulator cannot take a snapshot of the verifier's state (before making a try to guess its wanted edge) and set a "check point" for the simulation.
%\end{itemize}
%This combination results in a situation where if the simulator's guess was wrong for \emph{any of the iterations} of the core protocol, it needs to go back to the beginning of the first iteration, creating an exponential-time simulation, at least by classical rewinding technique.
%
%This problem was solved by Watrous, in his seminal work \cite{watrous2009zero}.
%The work presented a \emph{quantum rewinding technique} that, in a nutshell, enables a quantum simulator to amplify the amplitudes that the verifier's demanded edge and the simulator's guess correlate. This result was the first to show that classical protocols can be zero-knowledge against quantum attacks (by constructing the abovementioned quantum simulator for the \cite{goldreich1986prove} proof system).
%
%The quantum rewinding technique manages to eliminate the state cloning that happens during the naive simulator's snapshot, but uses a strong property of the protocol: very roughly, it rests upon the fact that the probability the simulator guesses correctly the edge demanded by the verifier is \emph{both} (1) a noticeable probability, and (2) independent of the inner quantum state of the verifier.
%Constant-round zero-knowledge protocols, which we discuss next, seem to require techniques of different nature.
%More specifically, in a sound protocol, the challenge space of the verifier is of exponential size, but in a many-round protocol this challenge space can be broken down into independent small challenges (e.g. in the core protocol we saw earlier, on each round the verifier randomly asks for one edge, which is not that hard to guess), making the probability of the simulator to guess correctly the challenge noticeable at each step.
%On the other hand, in a constant-round protocol the challenge space cannot be broken down to small challenges and the verifier's challenge cannot be guessed with a noticeable probability, and thus it seems that the above requirements of the quantum rewinding technique are too restricting for constant-round protocols with both zero-knowledge and negligible soundness error.
%
%
%
%
%
%
%\subsection{Constant-Round Zero-Knowledge and Extraction}\label{subsection:constant_round_and_extraction}
%As we explain next, constant-round zero-knowledge protocols are closely related to \emph{extraction} of information from circuits, and more specifically to \emph{extractable commitments}\footnote{For the sake of this technical overview we will speak about "extractable commitments" very informally. When we say "extractable commitment" we refer to a subprotocol that functions inside a zero-knowledge protocol (for NP), where the verifier can commit to a value (that is, the value is both hidden and cannot be changed after subprotocol has ended) and a simulator that has access to the verifier's circuit and inner state can extract the committed value and efficiently generate a transcript that's computationally indistinguishable from a real one.}.
%We show this connection by one example where extractable commitments enable a constant-round zero-knowledge protocol.
%
%Consider a \emph{parallel} repetition of the core protocol we saw earlier: The prover sends a stream of $\poly(|x|)$ (where $x$ is the protocol joint input, and instance from an \NP language $\lang$) commitments, $\alpha$ (thinking about the protocol from subsection \ref{subsection:intro_to_qzk}, this corresponds to sending commitments to a sequence of $\poly(|G|)$ legal 3-colorings each of them permuted), the verifier sends $\beta$, $\poly(|x|)$ challenges (one challenge for each committed permuted 3-coloring), and the prover sends $\gamma$, partial openings to the commitments $\alpha$ so that the challenge is answered (in our example, the prover shows that for each challenge $e$, that the wanted edge is colored legally).
%
%As we briefly discussed at the end of subsection \ref{subsection:intro_to_qzk}, a naive approach of challenge-guessing won't work here because the challenge space is huge, and one way to obtain a zero-knowledge protocol (and keep the number of rounds constant) is to somehow let the simulator know what $\beta$ is before it simulates $\alpha$, but also not let the prover in the protocol know this $\beta$ in advance (because if it knows $\beta$, the protocol won't be sound) - this is where extractable commitments can aid.
%Using extractable commitments, we can construct the following protocol: the verifier starts with giving an extractable commitment to $\beta$, the prover sends its commitments\footnote{For the actual protocol to be provably sound, the prover needs to give an extractable commitment, but we'll ignore this for now.} $\alpha$, the verifier opens the commitment to $\beta$, and the prover sends partial openings $\gamma$ to the commitments $\alpha$, so that the challenge $\beta$ is answered.
%
%\paragraph{Constant-Round Zero-Knowledge Protocols Against Restricted Quantum Verifiers.}
%In the classical setting, extractable commitments (and in particular constant-round zero-knowledge protocols) are known to exist given the existence of one-way functions.
%As it turns out, using very similar tools and assuming the existence of (quantum-secure) injective one-way functions, we can construct a toy example of an extractable commitment (and thus a constant-round zero-knowledge protocol) that's extractable from a very restricted form of verifiers, namely, \emph{non-aborting explainable quantum verifiers}.
%Informally, explainable verifiers, first introduced in \cite{bitansky2019weak}, are ones where every message they send is in the support of the honest verifier, and additionally, they can abort at any step of the protocol.
%For a classical-verifier protocol (as in our case, where both parties are classical algorithms) this means that when communicating with an explainable verifier (even a quantum one), at any step of the protocol there exists a string of random coins $r$ s.t. the transcript of the verifier so far can be generated by taking the honest classical verifier (with randomness $r$) and communicate with the prover's messages so far, and generate the current transcript (that is, the verifier's transcript can always \emph{be explained} by some string of randomness, until there was an abort, if there was).
%Non-aborting explainable verifiers are simply explainable verifiers that do not abort.
%\omri{Show the example of the extractable commitment, then the extraction procedure on it, and then the problem when aborts are added.}
%\omri{Possible side note is to explain why Watrous rewinding doesn't seem to help, but this might be too distracting.}
%
%
%
%
%
%\omri{End of paragraph, back to the subsection.}
%Quantumly-extractable commitments (where a quantum simulator that has access to the circuit of an arbitrary polynomial-size quantum verifier and inner quantum state can efficiently simulate the protocol) seem to require new properties over the ones needed from classically-extractable commitments:
%\begin{itemize}
%	\item
%	{\bf No-Cloning Extraction:}
%	The extraction needs to be cloning-free and the simulator cannot assume to copy the verifier's state at any point of the simulation.
%	More generally, we should aspire for a simulator that simulates the interaction "in a single pass", and uses the verifier's state only once for each of the steps of the protocol.
%	
%	\item {\bf Keeping the Verifier's Inner State:}
%	During simulation, the inner (quantum) state of the verifier that the simulator holds at the end of extraction should look like the verifier's regular inner state at the end of extractable commitment subprotocol, when it regularly interacts with the honest prover.
%\end{itemize}
%
%In simpler words, we want some special properties from our protocol in order to prove it quantum-secure.
%Sometimes, when we want to construct zero-knowledge protocols with special properties in the classical setting, it can be shown to be impossible to do with what's called a \emph{black-box simulator}.
%A black-box simulator is a ZK simulator that uses only oracle access to the verifier's input/output function, for example, the simulator we saw for the protocol from subsection \ref{subsection:intro_to_qzk} (both the core protocol and the many-rounds, sound protocol).
%On the other hand, a \emph{non-black-box simulator} is one that uses the fact that it actually has the verifier's circuit (and inner state), and can perform some clever operations using not only oracle access to the circuit, but the circuit itself.
%
%One famous example of a protocol with special properties that is proven to be both, impossible to construct by a black-box simulator and possible to construct by a non-black-box simulator is \omri{a few examples are given in Barak's paper. for example, constant-round zk with public coins.}
%To conclude, we aim for a protocol and simulation strategy that's non-restricting as possible, and thus we explore the possibility of non-black-box simulation to achieve a constant-round zero-knowledge protocol with postquantum security.
%
%
%
%
%
%
%
%
%
%
%%Recall the simulation from subsection \ref{intro:simulator}.
%%The reason $S$ made a guess to what was the verifier's demand, is so it can commit to the corresponding values that will make it possible to later open the commitment in a way that answers the challenge (i.e. in the specific case of the protocol from subsection \ref{intro:protocol}, answering the challenge means to show that the demanded edge is colored legally).
%%This notion captures a more general strategy in constructing zero-knowledge protocols: a way to build provable zero-knowledge protocols is to construct them such that the challenge of the verifier (in the example from subsection \ref{intro:protocol}, the challenge was the chosen edge the prover needs to open, and in the later version of the sound protocol, the challenge was all edges the verifier wanted the prover to open, over all $\poly(|E|)$ iterations) is hidden from the prover in the real interaction (so that the protocol is sound), but a simulator which has access to the verifier's code and inner state during interaction, can access the challenge, or make repeated and likely tries to guess it in advance {\bf before} the step in the protocol where the prover needs to commit to something that should answer the challenge.
%
%%The above observation yields a natural template for constant-round zero-knowledge protocols, using extractable commitments: the verifier starts with giving an extractable commitment to a \emph{string} of challenges $\beta$, the prover sends commitments\footnote{For the actual protocol to be provably sound, the prover needs to give an extractable commitment, but we'll ignore it for now.} $\alpha$ to a sequence of instances (thinking through the protocol from subsection \ref{intro:protocol}, this corresponds to sending commitments to a sequence of permuted graph legal 3-colorings), the verifier opens the commitment to $\beta$, and the prover sends $\gamma$, partial openings to the commitments $\alpha$ so that the challenge is answered (in our example, the prover shows that for each instance, the wanted edge is colored legally).
%
%%If the commitment scheme is indeed extractable the above protocol can be shown to be zero-knowledge, thus we currently focus on how to construct quantum-extractable commitments, that is, commitments s.t. if a \emph{quantum} sender manages to successfully commit (and this is something that can be checked publicly by both parties), then the extractor can extract the committed value.
%
%
%
%%\omri{remaining bullets:}
%%\begin{itemize}
%%	\item
%%	Current solution by Unruh - commitments that are extractable from non-aborting explainable senders.
%%	
%%	\item
%%	A toy exmaple of a construction inspired by Unruh's proofs of knowledge - a commitment scheme that is quantum-extractable from non-aborting explainable senders.
%%	
%%	\item
%%	We want to protect against aborters: problems with aborting adversaries in ZK settings, let alone in extractable commitments, where it simply makes the scheme not extractable.
%%	
%%	\item
%%	we need no-cloning extraction from explainable senders, they seem to pose a fundamental barrier in the quantum setting, and so in the classical setting.
%%	But, can we get it for them?
%%	
%%	\item
%%	In the classical setting, when we want ZK (or extraction) with some special properties, sometimes it is provably impossible to get them with black-box simulation.
%%	Famous example: It's impossible to prove that a constant-round public-coin protocol is zero-knowledge by a black-box simulation.
%%	
%%	\item
%%	Recall that we cannot clone, and we would like to aim for a strategy that will be as non-restricting as possible - a no-cloning extraction technique.
%%	We explore the possibility of performing a non-BB extraction, without cloning.
%%	
%%\end{itemize}
%
%
%
%
%
%
%
%
%
%
%\subsection{Cloning and Non-Black-Box Simulation in the Classical World}
%(Main goal of this subsection: a brief overview of existing non-BB techniques, explaining why they use cloning.)
%
%Bullets:
%\begin{itemize}
%	\item
%	Existing techniques might be non-BB, but still do cloning of verifier's state.
%	
%	\item
%	Barak's technique: Remarkably, not rewinding but still cloning.
%	
%	\item
%	Homomorphic trapdoor paradigm also uses cloning.
%\end{itemize}
%
%
%
%
%
%
%
%
%\subsection{Our No-Cloning Extraction Technique}
%We now turn to describing our no-cloning extraction technique.
%We saw earlier in subsection \ref{subsection:constant_round_and_extraction} that showing that a protocol is zero-knowledge against explainable quantum verifiers already seem like a challenge, thus it is an essential step to try and first build a protocol against explainable quantum verifiers.
%%Also observe that in the toy exmaple from subsection \ref{subsection:constant_round_and_extraction} it can be seen that we didn't even manage to simulate successful transcripts, that is, if the explainable verifier aborts at any step, the simulator's output can simply be $\bot$, and if the interaction ended successfully with no abort, the output is the verifier's inner quantum state.
%Our hope is that we can later bridge this gap to simulating fully malicious quantum verifiers, and as it will later turn out, indeed the problem of simulating explainable quantum verifiers captures an essence of this problem, and the gap can be bridged by combining already-existing techniques from the zero-knowledge realm.
%
%\paragraph{Aborts as a Tool for Verifiers to Descover Secret Information}
%As a side note, the only difference in the computational model of explainable verifiers, and the model we already showed quantum security for earlier (non-aborting explainable verifiers, in the toy protocol) is the aborts.
%\omri{If we would like to say something about the fact that aborting verifiers are dangerous, I think that this is a good place to do so. We can speak about something Nir mentioned about hard-core bits, and add that it might be plausible that over polynomially-many interactions, long secrets (like a witness!) can be revealed.}
%
%
%
%\medskip
%\omri{Back to the subsection:}
%Our intuition is to try and construct a protocol that is simulatable by a simulator that does a single pass over the interaction, without cloning the verifier's state.
%To furthermore simplify our thinking in this overview we currently think of the verifier as a classical circuit - we anyway set for ourselves the restriction of not cloning its (now classical) inner state during the simulation, and as we'll see, this strategy of no-cloning simulation will later easily translate to simulation of quantum verifiers.
%
%One (very general) template that could satisfy this no-cloning need is the following: The verifier will send a commitment to a message, and then send a challenge that is unsolvable by a possibly malicious prover, but is solvable by the simulator that has the verifier's state and circuit.
%After the verifier's challenge is sent, if the answer from the prover satisfies the challenge, the verifier will open the commitment to the message, and otherwise give no information.
%For the template to be a little more concrete, think of the challenge a an encryption of a uniformly random secret.
%\begin{enumerate}
%	\item
%	The verifier $\zkV$ sends $\cmt \gets \Com(m; r)$.
%	It then computes $t \gets U_\secp$ and sends $\ciph \gets \enc(t)$.
%	
%	\item
%	The prover $\zkP$ sends a guess $t'$.
%	
%	\item
%	$\zkV$ rewards a successful challenger: if $t = t'$ it outputs $r$, the opening for $\cmt$, otherwise nothing $\bot$.
%\end{enumerate}
%There are numerous problems with this template and explainable verifiers, but the main one is that even if the simulator will be able to know $t$ (which doesn't even seem to be the case), an explainable verifier can always decide to abort when it needs to answer a successful challenger.
%
%Our next template will be identical, but the protocol will let the verifier reward a successful challenger \emph{without knowing} if the challenger was successful or not, this will solve the earlier problem of the verifier aborting whenever it needs to reward a successful challenger.
%This can be done by using function-private secure function evaluation (SFE) when computing the verifier's response for the prover's try.
%\begin{enumerate}
%	\item
%	The verifier $\zkV$ sends $\cmt \gets \Com(m; r)$.
%	It then computes $t \gets U_\secp$ and sends $\ciph \gets \enc(t)$.
%	
%	\item
%	The prover $\zkP$ sends a guess $t'$ inside an SFE encryption $\ciph_{\zkP} \gets \sfeEnc(t')$.
%	
%	\item
%	$\zkV$ performs an SFE evaluation of its reward circuit (that outputs $r$ only for $t$ and $\bot$ otherwise): it sends to the prover $\evciph \gets \sfeEval\Big(\text{(The reward circuit of $\zkV$)},\, \ciph_{\zkP} \Big)$
%\end{enumerate}
%The above template solves the problem of the verifier not rewarding successful challengers, but it's still unclear how the simulator can get $m$.
%\omri{A note for us: motivation up to now is to get template for a protocol that enables a one pass for the simulator (and thus no cloning), given that the simulator succeeds in answering the verifier's challenge, which is the problem we solve next.}
%
%Thinking about non-black-box techniques, we recall the non-black-box technique from \cite{bitansky2019weak} - even though the technique itself used cloning and isn't usable in our quantum setting, we explore the more general idea of using the verifier's circuit in a non-black-box way, by performing a homomorphic evaluation of it to create the wanted asymmetry between the simulator and the prover.
%
%An observation that's important to our construction is that we might not know how to satisfy exactly the above template (e.g. in the last template the prover can't get $r$, which is good, but we don't know how to let the simulator get $r$), but we can use a combination of fully-homomorphic encryption (FHE) with non-black-box homomorphic evaluation of the verifier's circuit along with SFE, in order to get a goal that's close to what we described earlier: We are able to construct a no-cloning simulator that has an advantage over the prover (has an advantage, but doesn't yet knows how to get the message $m$).
%$\zkV$ can use FHE for the encryption of $t$, and the simulator can obtain an encryption of $r$, and because $\zkP$ can't get an encryption of $r$, the simulator has an advantage.
%More precisely, the simulator $\zkS$ can obtain a FHE encryption of $r$ in the following way:
%\begin{enumerate}
%	\item
%	$\zkS$ will take the verifier's encryption of $t$, $\ciph = \fheE(t)$, and perform homomorphic evaluation of its SFE encryption to get $\fheE(\sfeEnc(t))$.
%	
%	\item
%	$\zkS$ uses $\zkV$'s circuit to perform a homomorphic evaluation of $\zkV$'s reponse to get $\fheE(\sfeEnc(r))$.
%	
%	\item
%	Finally, $\zkS$ performs a third and final homomorphic evaluation for its SFE decryption circuit, to get $\fheE(r)$.
%\end{enumerate}
%More generally, the idea is that the when the verifier uses FHE to encrypt its random secret, the simulator can turn an encryption of one secret $t$, to an encryption of another secret $s$.
%
%A natural question is to now ask: How can we use the simulator's ability to transform one secret to another, in order for it to know $m$?
%We first notice that a program that simply checks if its input is an encryption of some secret $s$, and rewards you with the message $m$ if the input is indeed such an encryption, is a very restricted kind of program called \emph{Compute-and-Compare} (CC).
%CC programs are programs that execute a function $f$ on their input $x$, and if $f(x)$ equals one, specific target $y$, then they output a messsage $a$, and output $\bot$ if $f(x) \neq y$.
%Such a program is usually denoted $\oCC\big[ f(\cdot), y, a \big]$.
%For CC programs we have the cryptographic tool of CC obfuscation, which provides complete hiding of $f$ and $a$ when $y$ is chosen uniformly at random.
%
%The above tool gives us a way to both let the simulator obtain $m$ and hide $m$ from the prover, all of this in one simulator pass:
%Imagine that the verifier now chooses \emph{two} random secrets; a random target $t$ which it encrypts and sends to the prover, and a random target $s$ s.t. if the prover sends $t$ (as the prover's try, under SFE encryption), then the verifier responds with $s$ (under SFE evaluation).
%The verifier will send, along with the encryption of $t$ a CC obfuscation of the circuit $\oCC\big[ \fheD(\cdot), s, m \big]$, that rewards $m$ for an encryption of $s$.
%By the security of the CC obfuscation, because $s$ is chosen uniformly at random, information on the decryption circuit $\fheD$ of the FHE (that includes the $\fhe$ secret decryption key) and $m$ is completely hidden.
%\begin{enumerate}
%	\item
%	$\zkV$ computes $s \gets U_{\secp}, t \gets U_{\secp}$, and sends
%	$$
%	\ciph_{\zkV}\gets \fheE(t), \enspace
%	\obfC \gets \Obf\Big(\oCC\big[ \fheD(\cdot), s, m \big]\Big)\enspace .
%	$$
%	
%	\item
%	$\zkP$ computes its guess $t' \gets U_\secp$, and sends an SFE encryption of it $\ciph_{\zkP} \gets \sfeEnc(t')$.
%	
%	\item
%	$\zkV$ sends $\evciph \gets \sfeEval\Big(\oCC\big[ \mathsf{Id(\cdot)}, t, s \big],\, \ciph_{\zkP} \Big)$, where $\mathsf{Id(\cdot)}$ is the identity function.
%\end{enumerate}
%
%There is a new, small problem with our above structure: Malleability.
%More precisely, we don't know how the SFE and FHE schemes are implemented, and it could be the case that they are implemented by very similar, or at least structurally-connected algorithms, s.t. there's an efficient algorithm that turns an FHE encryption of $t$ to an SFE encryption of $t$, letting a malicious prover cheat the honest verifier (at the very least, it's unclear how to prove that it cannot be the case).
%
%A first step to overcome this problem is by making the prover first commit to the decryption key of its SFE encryption - it cannot know both how to turn $\fheE(t)$ to $\sfeEnc(t)$, and also how to decrypt $\sfeEnc(t)$, because that would be like breaking the security of the FHE\footnote{In order for this to work, the prover will later need to somehow prove that it behaved well and actually used the committed $\sfedk$ for its try under the SFE encryption, and this can be done by the same tools that will let us move from explainable to malicious verifiers, so we can assume that a malicious prover behaves well, in some restricted sense.}.
%This by itself seem to be insufficient in order to formally prove soundness, as the prover needs to give an actual \emph{quantumly-extractable} commitment for $\sfedk$ - but this takes us back to our initial goal, so we need to think of a different way to obtain the SFE key of a malicious prover.
%
%A valueble observation is that in the simulation example above, the simulator can compute its SFE key $\sfedk$ at any point before the point it actually computes it in the example, and in particular, can compute it before the protocol starts and commit to it already at the beginning of the protocol as a first prover message, note that such first message does not depend on any of the verifier's messages.
%If the first protocol message is by the prover and does not depend on verifier messages, by an averaging argument, we can always w.l.o.g. look only on non-uniform provers that send a deterministic first message (we consider n.u. provers by default, and in the quantum case, these provers should be n.u. with quantum advice, to capture the prover's inner quantum state in such averaging argument), in our case, if the message by a malicious prover is always the same then so is the committed $\sfedk$.
%
%At this point, we can use a non-uniformity trick in order to prove soundness: We use non-uniform advice in order to know what is the prover's committed key $\sfedk$ inside the commitment, that is, if there's a malicious prover $\zkP'$ that manages to transform $\fheE(t)$ to $\sfeEnc_{\sfedk}(t)$ (where $\sfedk$ is the SFE key it was committed to in the beginning), then there's a non-uniform prover $\zkP''$ that can break the security of the FHE encryption.
%
%\paragraph{From Non-Cloning Simulation of Classical Explainable Verifiers to Quantum Explainable Verifiers.}
%We now go back to thinking about quantum explainable verifiers (rather than classical explainable verifiers).
%The no-cloning simulation strategy described for classical explainable verifiers leaves a few small gaps, and one that's a bit more serious, in order to simulate quantum explainable verifiers.
%\begin{itemize}
%	\item
%	When the verifier encrypts its secret target $t$ it uses \emph{quantum} fully-homomorphic encryption (QFHE) rather than classical FHE.
%	
%	\item
%	Note that when the simulator performs the (now quantum) homomorphic evaluation of the circuit $\zkV$ it needs to also encrypt the verifier's inner quantum state, thus we use a public-key QFHE and the verifier will also send the public key, letting the simulator encrypting the inner state of $\zkV$ to perform the evaluation.
%	
%	\item
%	After the third homomorphic evaluation by $\zkS$ it holds $\qheE_{\qhepk}(s), \qheE_{\qhepk}(\ket{\psi})$, where $\ket{\psi}$ is the verifier's inner quantum state after performing its second step in the protocol.
%	$\qheE_{\qhepk}(s)$ is a classical ciphertext that can be encrypted as before by the CC obfuscated program $\obfC$, but $\ket{\psi}$ stays locked under the encryption.
%	This can be solved by adding the reward $\qhesk$ (the QFHE secret decryption key) to $m$ (in the third and last parameter of $\obfC$).
%\end{itemize}
%The more serious gap is created because the verifier can abort on its response step, after the simulator already encrypted the verifier's inner state - at that point the simulator is stuck with an encrypted state it cannot output, and the state is effectively lost.
%In these cases where the verifier aborts and the simulator is stuck, we would like to sample a transcript s.t. the verifier aborted, where we don't even try to do the extraction.
%sampling such transcript turns out as a non-trivial task to do in expected polynomial time, and the reason is mainly that it might be the case that the probability that the verifier aborts is negligible, making it hard to sample an aborting transcript.
%This can still be done in expected polynomial time, adjusting techniques first introduced in \cite{goldreich1996construct} to our setting. \omri{Should we say something more about this?}
%
%\paragraph{From Quantum Explainable Verifiers to Quantum Malicious Verifiers.}
%\omri{Needs a very brief and high-level explanation that there are existing techniques (citation: by who?), using constant-round WI proofs, that can reduce the problem of ZK against malicious verifiers to the problem of explainable verifiers.}


































\section{Restricted Quantum-Extractable Commitments}\label{sec:r_qex}
\omri{After writing body and intro, fix this small intro.}
Our no-cloning extraction technique will be used to construct numerous cryptographic functionalities, thus we aim to capture it by a single cryptogrpahic primitive that will be repeatedly used throughout the paper.

We call the cryptographic primitive that we use a \Name (\short in short), which is an interactive commitment scheme (with a constant number of communication rounds) with the usual binding and hiding, and an additional guarantee that there is some extraction algorithm $\Ext$ that for any efficient quantum sender, if the sender acts in an {\bf explainable} manner during interaction (being explainable is a weaker adversarial model, which we define next - hence the "restricted" in the primitive's name) and manages to successfully commit to something with a probability $p$, then with probability negligibly close to $p$, using the circuit of the sender and its quantum inner state, $\Ext$ will output the committed value and also the inner quantum state of the sender after interaction with the honest receiver.

\short is the main tool we use to construct classical constant-round QZK arguments for NP.
Later in the paper, by combining \short and the QZK arguments for NP we construct quantum-extractable commitments (QEX), that is, extractable for arbitrary efficient quantum senders (without the restriction that the sender has to be explainable).
We now define explainable senders and \short commitments.

\begin{definition}[Interactive Commitment]
	An interactive commitment scheme $(\comS, \comR, \decom)$ comprises two interactive \PPT algorithms $\comS, \comR$ and an additional deterministic polynomial-time algorithm $\decom$, with the following syntax:
	\begin{itemize}
		\item $\comS(1^{\secp}, x):$
		The sender $\comS$ takes as input a (public) security parameter $\secp \in \Nat$ and a bit string $x \in \{ 0, 1 \}^*$. It interacts with $\comR$ (a constant number of messages) to generate the transcript $T$.
		
		\item $\comR(1^{\secp}):$
		The receiver $\comR$ takes as input a security parameter $\secp \in \Nat$ and interacts with the sender. After having the interaction transcript $T$, it decides (by a public deterministic algorithm) whether to accept or reject the commitment by outputting a bit $\view_{\comR}\prot{\comS}{\comR}$.
		A malicious receiver $\commR$ may have an arbitrary output for $\view_{\commR}\prot{\comS}{\commR}$.
		
		\item $\decom(1^\secp, x, r, T):$ After successful commitment, $\comS$ can decommit to $x$ by sending $\comR$ a string $r$ (and also $x$).
		$\comR$ can validate the decommitment by checking whether $\decom(1^\secp, x, r, T) = 1$.
	\end{itemize}
	The scheme satisfies the following properties:
	\begin{enumerate}
		\item {\bf Perfect Binding:}
		Let $\commS = \{ \commS_{\secp} \}_{\secp \in \Nat}$ be any non-uniform unbounded sender, and let $T \gets \langle \commS \leftrightarrows \comR(1^\secp) \rangle$ be a transcript of an interaction such that $\view_{\comR}\prot{\commS}{\comR(1^\secp)} = 1$.
		Then, 
		$$
		\nexists x_1, r_1, x_2, r_2 \in \{ 0, 1 \}^*: x_1 \neq x_2, \,
		\decom(1^\secp, x_1, r_1, T) = 1, \, \decom(1^\secp, x_2, r_2, T) = 1 \enspace .
		$$
		
%		we have the following probability over the receiver's random coins:
%		$$
%		\forall \secp \in \Nat: \Pr\left[
%		A
%		\land
%		B
%		\pST
%		T \gets \langle \commS \leftrightarrows \comR(1^\secp) \rangle
%		\right] \leq \mu(\secp) \enspace ,
%		$$
%		where,
%		\begin{gather*}
%			A \equiv \left( \view_{\comR}\prot{\commS}{\comR(1^\secp)} = 1 \right) \enspace ,\\
%			B \equiv \left( \exists x_1, r_1, x_2, r_2 \in \{ 0, 1 \}^*: (x_1 \neq x_2), \,
%			\decom(1^\secp, x_1, r_1, T) = 1, \, \decom(1^\secp, x_2, r_2, T) = 1 \right) \enspace .
%		\end{gather*}
		
		\item {\bf Quantum Computational Hiding:}
		For any non-uniform polynomial-size quantum receiver $\commR = \{ \commR_\secp \}_{\secp \in \Nat}$ and any two sequences of length-$\ell(\secp)$ inputs $\{ x_\secp \}_{\secp \in \Nat}, \{ y_\secp \}_{\secp \in \Nat}$ we have,
		$$
		\{ \view_{\commR}\prot{\comS(1^\secp, x_\secp)}{\commR_\secp} \}_{\secp \in \Nat}
		\approx_c
		\{ \view_{\commR}\prot{\comS(1^\secp, y_\secp)}{\commR_\secp} \}_{\secp \in \Nat} \enspace ,
		$$
		where the view of an interactive quantum machine is the machine's inner state, which can in particular capture the classical transcript of an interaction.
	\end{enumerate}
\end{definition}

\subsection{Explainable Senders}
Explainable senders are a slightly weaker adversarial model than arbitrary malicious senders, defined (as explainable verifiers, in the context of ZK) in \cite{bitansky2019weak}.
Roughly speaking, explainable senders are senders whose messages are always in the support of the honest sender's messages, regardless of how the receiver’s messages are generated. We also allow such senders to abort at any stage of the interaction.
We

\begin{definition}[Explainable Transcript]
	Let $(\comS, \comR, \decom)$ be an interactive commitment scheme, and let $T$ be a transcript of messages between two arbitrary algorithms.
	We say that the transcript $T$ is explainable for security parameter $\secp \in \Nat$ (or just explainable), if there exists honest sender coins $r$ and a string $x$ such that $T$ can be generated by taking the receiver messages in $T$ and use them to interact with $\comS(1^\secp, x;r)$, until the point in $T$ that the sender aborts.
\end{definition}

Our commitment schemes will have the following useful trait.
\begin{definition}[Restricted Density]
	Let $(\comS, \comR, \decom)$ be an interactive commitment scheme, and let $T$ be a transcript of messages between two arbitrary algorithms.
	The scheme has restricted density, if whenever $T$ is accepted by the receiver and also is explainable, then it can be decommitted for some value, that is, there exist $x, r$ s.t. $\decom(1^\secp, x, r, T) = 1$.
\end{definition}

A restricted quantum-extractable commitment is an interactive commitment scheme where we have the guarantee that for any polynomial-size quantum sender, if the sender's transcript is explainable and succeeds with some probability to convince the receiver that it have committed successfully, then with probability almost as good, there is an extractor that can use the sender's circuit to extract the committed value, along with the transcript of the interaction (with the honest receiver) and its inner quantum state.

We consider this extraction to be restricted, because we can guarantee it only when the transcript is explainable, which is something that the receiver cannot efficiently check by itself.
Later in the paper we'll see how we can remove this restriction, and condition only on the acceptance of the receiver.

\begin{definition}[Restricted Quantum-Extractable Commitment]\label{def:r_qex}
	An interactive commitment scheme $(\comS, \comR, \decom)$ (with restricted density) is a restricted quantum-extractable commitment (or \short commitment) if there exists a \QPT algorithm $\Ext$ with the following syntax:
	\begin{itemize}
		\item 
		$(T, \ket{\phi}, x)\gets \Ext(\commS_\secp(\rho_\secp)):$ $\Ext$ gets as input a sender's circuit and inner quantum state, and outputs a tuple of transcript $T$, inner quantum state $\ket{\phi}$ and committed value $x$ (that under some conditions, should mimic a transcript and inner state generated by interaction of the sender with the honest receiver, plus a value the sender was maybe committed to).
	\end{itemize}
	For any quantum polynomial-size sender $\commS = \{ \commS_\secp(\rho_\secp) \}_{\secp \in \Nat}$ the following holds.
	\begin{itemize}
		\item {\bf Extractor Interaction Indistinguishability:}
		There exists an interactive (unbounded) machine $\comR^{\Ext(\commS)}$ such that the sender's view when interacting with it versus interacting with the honest receiver is computationally indistinguishable, 
		$$
		\{ \view_{\commS}\prot{\commS_\secp(\rho_\secp)}{\comR^{\Ext(\commS_\secp)}} \}_{\secp \in \Nat}
		\approx_c
		\{ \view_{\commS}\prot{\commS_\secp(\rho_\secp)}{\comR(1^\secp)} \}_{\secp \in \Nat} \enspace .
		$$
		
		\item {\bf Restricted Extraction:}
		For every $\secp \in \Nat$ denote,
		$$
		p_\secp := \Pr\left[ 
		\text{ $\comR(1^\secp)$ accepts $T$, and $T$ is explainable }
		\pST
		T \gets \langle \commS_\secp(\rho_\secp) \leftrightarrows \comR^{\Ext(\commS_\secp)} \rangle
		\right] \enspace ,
		$$
		then with probability $1 - p_\secp$, the transcript from the tuple $\Ext(\commS_\secp(\rho_\secp))$ outputs is not explainable, and with probability $p_\secp$, the output of $\Ext(\commS_\secp(\rho_\secp))$ is a sample from the distribution $D$ which satisfies,
			$$
			\{ D_\secp \}_{\secp \in \Nat}
			\approx_s
			\{ (T, \ket{\phi}, x) \}_{\secp \in \Nat} \enspace ,
			$$
			where the distribution $(T, \ket{\phi}, x)$ is defined as follows.
			Consider the distribution $(T', \ket{\phi'}, x')$ generated by interaction $T' \gets \langle \commS(\rho) \leftrightarrows \comR^{\Ext(\commS_\secp)} \rangle$, $\ket{\phi'}$ is the inner quantum state of $\commS$ at the end of interaction, and $x'$ is defined if $T'$ can be decommitted for it, otherwise it's $\bot$.
			Then $(T, \ket{\phi}, x)$ is the conditional distribution of that distribution, conditioned on $T$ being explainable and acceptable.
	\end{itemize}

	Additionally, the extraction is classicality preserving:
	\begin{itemize}
		\item 
		If the sender $\commS$ is a classical circuit then $\Ext(\commS)$ can be implemented by a \PPT algorithm.
	\end{itemize}
\end{definition}
\omri{(1) Add a syntax section to the definition - the extractor outputs a tuple or $\bot$, outputting a tuple doesn't say the extraction was successful. (2) the transcript and quantum state are computationally indistinguishable from the of the ones ofthe real interaction, not including the committed value x.
(3) Do we need to add a comment that the computational indistinguishability holds only when $p$ is noticeable?}
\omri{It is correct to say that with probaility $1 - q$, if the extractor outputs a tuple, then the transcript is not explainable: this follows from the observation that if the extractor failed to extract an explainable transcript, it could have been only because the verifier aborted in the homomorphic evaluation, and thus the extractor will output $\bot$ and not the transcript.}
\omri{interaction + quantum state of extraction interaction is computationally indistinguishable. The extraction suffices: with probability $p$ that the sender is explainable it samples from the conditional distribution, with probability $1 - p$, if outputs transcript and state, transcript is not explainable.}


\iffalse
\paragraph{Comments about the definition.}
\begin{itemize}
	\item 
	The extractor in the above definition is a natural extension of what extractors usually output - it does not output only the committed value, but importantly (in the quantum interactive setting) also the inner quantum state of the sender, after the interaction with the honest receiver.
	\item 
	We diverge from our convention of security that by default considers n.u. quantum circuits without quantum advice, because this definition is more natural to be defined with quantum advice, which usually captures the sender's inner quantum state in an interactive setting.
	Below we also provide a definition for extraction from senders without an initial quantum advice (and thus such definition uses slightly weaker hardness assumptions, that is, security of primitives in the construction should hold against quantum adversaries without quantum advice rather than with it).
	As far as we know, it will still enable similar security reductions and extraction.
	\omri{Decide ones and for all what is the course of displaying the commitments: (1) with advice and then correction in ZK to non-advice, or (2) non-advice from the beginning.}
%	It is worth noting that the definition could be also defined to extract from senders without an initial quantum advice (and such definition assumes security only for regular efficient n.u. quantum circuits), and as far as we know, it will still enable similar security reductions and extraction. \omri{Note where, where later in this section, there is an example of how we would use it without advice. This should appear as paragraph under the ZK proof.}
\end{itemize}


\omri{VERSION 2, without quantum advice, below.}
\begin{definition}[Restricted Quantum-Extractable Commitment]
	An interactive commitment scheme $(\comS, \comR, \decom)$ is a \Name (or, a \short commitment) if there exists a \QPT algorithm $\Ext$ with the following properties:
	Let $(\mathsf{P_1}, \mathsf{P_2})$ be two interactive efficient (possibly quantum) circuits $\POne = \{ \POne_{, \secp} \}_{\secp \in \Nat}, \PTwo = \{ \PTwo_{, \secp} \}_{\secp \in \Nat}$ that end their interaction with the subprotocol $(\commS, \comR)$, then the following holds.
	For every $\secp \in \Nat$ denote,
	$$
	p_\secp := \Pr\left[ 
	\left(  \view_{\comR}\prot{\commS_\secp}{\comR(1^\secp)} = 1
	\right) \land
	\left( 
	\text{$T_{(\commS, \comR)}$ is explainable}
	\right)
	\right] \enspace ,
	$$
	then there's a probability $q_\secp$ and a negligible function $\mu(\cdot)$ s.t. for every $\secp \in \Nat$, $\abs{q_\secp - p_\secp} \leq \mu(\secp)$ and with probability $q_\secp$ we have:
	\begin{itemize}
		\item {\bf Restricted Density:}
		The transcript is indeed decommitable, that is, there exist $x, r$ s.t. \newline$\decom(1^\secp, x, r, T) = 1$.
		
		\item {\bf Restricted Extraction:} We have,
		$$
		\{ \langle \mathsf{P_{1, \secp}} \leftrightarrows \mathsf{P_{2, \secp}} \rangle^{\Ext(\commS_{\secp})} \}_{\secp \in \Nat}
		\approx_c
		\{ (T, \ket{\phi}, x) \}_{\secp \in \Nat} \enspace ,
		$$
		where the distributions above are defined as follows:
		\begin{itemize}
			\item $\langle \mathsf{P_{1, \secp}} \leftrightarrows \mathsf{P_{2, \secp}} \rangle^{\Ext(\commS_{\secp})}:$
			Consider the process of interaction between $\mathsf{P_1}, \mathsf{P_2}$, where in the end, instead of communication through $\commS_\secp, \comR(1^\secp)$, we execute $\Ext$ on the circuit $\commS_\secp$, the inner quantum state $\ket{\psi}$ of $\mathsf{P_1}$, and the transcript so far.
			We output the output of $\Ext$.
			
			\item $(T, \ket{\phi}, x):$
			Consider the distribution $D = (T', \ket{\phi'}, x')$ generated by interaction between $\POne, \PTwo$ (including $(\commS, \comR)$ in the end); $T'$ is the transcript, $\ket{\phi'}$ is the inner quantum state of $\POne$ at the end of interaction, and $x'$ is defined if it is the only value $T_{(\commS, \comR)}$ can be decommitted for, otherwise it's $\bot$.
			Then $(T, \ket{\phi}, x)$ is the conditional distribution of $D$, conditioned on $T_{(\commS, \comR)}$ being explainable and accepting, and decommits only to $x$.
		\end{itemize} 
	\end{itemize}
	With probability $1 - q_\secp$, $\langle \mathsf{P_{1, \secp}} \leftrightarrows \mathsf{P_{2, \secp}} \rangle^{\Ext(\commS_{\secp})}$ just outputs $\bot$.
	Additionally, the extraction is classicality preserving:
	\begin{itemize}
		\item 
		If the sender $\commS$ is a classical circuit then $\Ext(\commS)$ can be implemented by a \PPT algorithm.
	\end{itemize}
\end{definition}
\fi





\omri{TO DO: Make sure you also output the transcript $T$ by decrypting the homomorphic encryption and encrypting it with the SFE.}

\medskip
We now show our construction of \short commitments.

\paragraph{Ingredients and notation:}
\begin{itemize}
%	\item 
%	A non-interactive commitment scheme $\Com$.
	\item 
	A CC obfuscator $\Obf$.
	\item 
	A quantum fully homomorphic encryption scheme $(\qheG, \qheE, \qheQE, \qheD,\newline \qheQD, \qheEv )$.
	\item
	A 2-message function-hiding secure function evaluation scheme $(\sfeGen,$ $\sfeEnc,$ $\sfeEval,$ $\sfeD)$.
\end{itemize}


We describe the protocol in \figref{fig:r_qex_commitment}.
\omri{Comments about:
	(1) We lose access to the quantum state and thus the ZK is only w/out advice. could be fixed by a property of the QEX commitment.
	(2) The fact that we don't have to have security against quantum advice to do reductions wit the scheme in the middle of the }

\protocol
{\proref{fig:r_qex_commitment}}
{A classical 3-message restricted quantum-extractable commitment scheme.}
{fig:r_qex_commitment}
{
	\begin{description}
		\item[Common Input:] $1^\secp$, the security parameter $\secp \in \Nat$ in unary.
		\item[$\comS$'s private input:] a string $\ins \in \{ 0, 1 \}^*$.
	\end{description}
	
	\begin{enumerate}
%		\item
%		{\bf Coin Tossing Into the Well:} 
%		$\comS$ computes $r_{\comS} \gets U_{p(\secp)}$ (where $p(\cdot)$ is a polynomial that denotes the amount of randomness the sender uses for the rest of the interaction), and sends a non-interactive commitment to that randomness $\cmt_{\comS}\gets \Com(r_{\comS})$.
%		Then, $\comR$ sends a random string $r_{\comR} \gets U_{p(\secp)}$.
%		
%		\item 
%		{\bf Quantum-Extractable Procedure by the Sender:} The parties interact in order for $\comS$ to commit for $\ins$, where $\comS$ uses the randomness $r = r_\comS \oplus r_\comR$.
%		\begin{enumerate}
		\item 
		$\comS$ computes $s \gets U_{\secp}, t \gets U_{\secp}, (\qhepk, \qhesk) \gets \qheG(1^{\secp})$ and sends
		$$
		\qhepk, \enspace
		\ciph_{\comS}\gets \qheE_{\qhepk}(t), \enspace
		\obfC \gets \Obf\Big(\oCC\big[ \qheD_{\qhesk}(\cdot), s, (\qhesk, \ins) \big]\Big)\enspace .
		$$
		\item \label{receiver_response}
		$\comR$ computes $\sfedk \gets \sfeGen(1^\secp)$, and sends $\ciph_{\comR} \gets \sfeEnc_{\sfedk}(0^\secp)$.
		\item \label{sender_response}
		$\comS$ sends $\evciph \gets \sfeEval\Big(\oCC\big[ \mathsf{Id(\cdot)}, t, s \big],\, \ciph_{\comR} \Big)$, where $\mathsf{Id(\cdot)}$ is the identity function.
		\item {\bf Acceptance:}
		$\comR$ accepts if the sender did not abort during the protocol.
		
	\end{enumerate}
}

\begin{itemize}
	\item $\decom(1^\secp, x, r, T):$
	To decommit, we basically check that $T$ can be generated by the given input.
	more specifically, we verify that $T$ is consistent with an execution of $\comS(1^\secp, x ;r)$.
\end{itemize}

\subsection{Binding and Hiding of the Scheme}
We explain why the above scheme is binding and hiding.
\begin{claim}
	The interactive commitment scheme described in \proref{fig:r_qex_commitment} is perfectly binding.
\end{claim}
\begin{proof}
	This basically follows from the fact that the obfuscator outputs a correct program with probability 1.
	
	More formally, assume towards contradiction that there's a sender $\commS$ (and security parameter $\secp \in \Nat$, not even a need for asymptotics here) that breaks binding,
	so after it interacts with $\comR(1^\secp)$, there's two possible openings: 
	$$
	x_1 \neq x_2, \,
	\decom(1^\secp, x_1, r_1, T) = 1, \, \decom(1^\secp, x_2, r_2, T) = 1 \enspace .
	$$ 
	This in particular means that the obfuscated CC program in the transcript can output both $x_1$ and $x_2$, in contradiction.
%	 so there's a non-zero probability $\varepsilon(\secp)$ s.t. for infinitely many $\secp \in \Nat$, $\commS$ convinces $\comR$, but can decommit to some two values $x_1, x_2, x_1\neq x_2$.
%	This means (due to the perfect binding of the non-interactive commitment that $\commS$ gives) that for uniformly random coins $r_3$ for the CC obfuscator, with a noticeable probability there are strings $\qhesk, s, \qhesk', s'$,
%	$$
%	\Obf\Big(\oCC\big[ \qheD_{\qhesk}(\cdot), s, (\qhesk, \ins_1) \big] ; r_3\Big) =
%	\Obf\Big(\oCC\big[ \qheD_{\qhesk'}(\cdot), s', (\qhesk', \ins_2) \big] ; r_3\Big) \enspace ,
%	$$
%	which in particular implies that with a noticeable probability, the CC obfuscator outputs an incorrect program, which in turn contradicts the fact that the obfuscator outputs a correct program with overwhelming probability.
\end{proof}


\begin{claim}
	The interactive commitment scheme described in \proref{fig:r_qex_commitment} is quantum computationally hiding.
\end{claim}
\begin{proof}
	\omri{Two hybrids: (1) just change $s$ in the SFE evaluation. (2) just change $x_1$ to $x_2$ in the CC obfuscation - this yields an averaging argument, followed by using the CC obfuscation security.}
	The hiding property follows from the security of the QHE, the security of the CC obfuscator and the circuit privacy of the SFE, and will be proved by a hybrid argument.
	Let $\commR = \{ \commR_\secp \}_{\secp \in \Nat}$ be an efficient
	Fix 
\end{proof}










	
%\subsection{Quantum Zero-Knowledge}
%We construct a simulator $\zkS$ that for every quantum verifier $\zkmV$, simulates an output distribution that is computationally indistinguishable from the output distribution of $\zkmV$ after interaction with the honest prover.
%%	The simulator $\zkS$ has expected polynomial time and is non-black-box in the sense that it will make use of the fact that it has the circuit of $\zkmV$ (rather than only oracle access to it).
%%As part of the simulation we will need to resolve an issue with simulating abort distributions and stay in expected polynomial time, for this we use techniques similar to \cite{goldreich1996construct}, with slight modifications.
%%	The running time of the simulator is expected polynomial time, and will suffice a stronger guarantee of "almost strict polynomial time", that is, there is a fixed polynomial s.t. with overwhelming probability the simulator's running time does not surpass it.
%
%\noindent {\bf Note:} As a convention for the simpicity of describing $\zkS$, in each part of the following simulation except part \ref{qhe_simulation}, whenever we execute $\zkmV$'s circuit it is implicitly possible (and will not be noted every time) that the output message is an abort ($\bot$). In this case the simulator halts simulation and outputs the inner quantum state of $\zkmV$.
%The simulator's behaviour on an abort in part \ref{qhe_simulation} is explicitly described in part \ref{check} of the simulation.
%
%\medskip
%\paragraph{$\zkS(\ins,\zkmV_\secp):$}
%\begin{enumerate}
%	\item {\bf Simulation of Coin Tossing and 1st step of $\zkmV$'s Extractable Commitment:}
%	Execute the first message generation of $\zkmV$ to get a commitment to $r_{\zkmV}$, then execute the response of the prover $r_\zkP \gets U_{p(\secp)}$.
%	Execute the first message of $\zkmV$ in the second stage of the protocol and obtain $(\ciph_{\zkmV} \gets \qheE_{\qhepk}(t), \; \qhepk, \; \obfC)$, and the quantum inner state $s_{\zkmV}$ of $\zkmV$.
%	
%	\item  {\bf Quantum Homomorphic Evaluation of $\zkmV$'s Response:}
%	Now comes the non-black-box part of the simulation.
%	\begin{enumerate}
%		\item 
%		Compute $\sfedk \gets \sfeGen(1^\secp)$ and homomorphically evaluate the circuit $\sfeEnc_{\sfedk}(\cdot)$ on $\qheE_{\qhepk}(t)$ to obtain a classical ciphertext $\qheE_{\qhepk}(\sfeEnc_{\sfedk}(t))$.
%		\item 
%		Using $\qhepk$, encrypt the quantum inner state of $\zkmV$ to obtain $\qheQE_{\qhepk}(s_{\zkmV})$.
%		\item  \label{qhe_simulation}
%		Homomorphically evaluate $\zkmV$ on the (concatenated) ciphertext
%		$$
%		\qheE_{\qhepk}(\sfeEnc_{\sfedk}(t)),\qheQE_{\qhepk}(s_{\zkmV}) \enspace ,
%		$$
%		to obtain $\mathbf{\hat{c}}$, a classical encryption of the output message of $\zkmV$ (which can also be an abort $\bot$), and $\ket{\Phi}$, a quantum encryption for its inner quantum state.
%	\end{enumerate}
%	
%	\item {\bf Validity Check, then Abort Simulation or Extraction:}
%	\begin{enumerate}
%		\item 
%		$\mathbf{\hat{c}}$ is a homomorphic encryption of either $\bot$ or $\sfeEnc_{\sfedk}(s)$, thus homomorphically evaluate the SFE decryption circuit $\sfeD_{\sfedk}(\cdot)$ on the ciphertext to get a homomorphic encryption $\mathbf{\hat{c}'}$ of either $s$, or some other arbitrary string.
%		\item \label{check}
%		Compute $\obfC(\mathbf{\hat{c}'})$, if it is $\bot$ then discard all information kept until now and execute $\zkSA(\ins, \zkmV)$, otherwise we have $\obfC(\mathbf{\hat{c}'}) = (\qhesk, \beta)$.
%		Use $\qhesk$ to compute $s'_{\zkmV} = \qheQD_{\qhesk}(\ket{\Phi})$, the verifier's inner state after stage \ref{verifier_response} of the protocol.
%	\end{enumerate}
%	
%	\item {\bf Simulation of Sigma Protocol Messages:}
%	Use the simulator $\SigS$ (from the special ZK property of the sigma protocol) to compute $(\alpha, \gamma) \gets \SigS(\ins, \beta)$.
%	Compute $\zkmV$'s response for the message $\alpha$ (it is either $\beta$ or an abort $\bot$), and answer with $\gamma$.
%	Conclude simulation by outputting the verifier's inner state.
%\end{enumerate}
%
%
%
%
%
%\medskip
%\paragraph{$\zkSA(\ins,\zkmV_\secp)$:}
%\begin{enumerate}
%	\item {\bf Estimation of Probability to Abort in Simulated Transcript:}
%	Iterate until either there are $\secp^2$ aborts, or $2^\secp$ iterations have passed:
%	execute $\zkS$ until (and not including) stage \ref{check}, then, only if $\obfC(\mathbf{\hat{c}'}) = \bot$ (and there wasn't an abort in an earlier stage in this iteration) count it as an abort.
%	
%	If you exitted the loop because you ran for $2^\secp$ iterations, halt and output $\zkFail$.
%	Otherwise, let $N$ denote the number of iterations ($N$ is a random variable), and set $a'(\ins) = \frac{\secp^2}{N}$.
%	
%	\item {\bf Attempt to Get a Valid Abort Transcript:}
%	Iterate until either you get an abort, or $\secp\cdot \ceil{\frac{1}{a'(\ins)}}$ iterations have passed:
%	simulate the protocol honestly (simulate the honest prover, and get responses from $\zkmV$ by using its circuit as a black box) until and including stage \ref{verifier_response}.
%	If $\zkmV$ responded with $\bot$ (and there wasn't an abort in an earlier stage of this iteration) count it as an abort.
%	
%	If you exitted the loop because you ran for $\secp\cdot \ceil{\frac{1}{a'(\ins)}}$ iterations, halt and output $\zkFail$.
%	Otherwise, halt and output $\zkmV$'s inner state.
%\end{enumerate}
%
%\noindent 
%\paragraph{Overview of the Simulation.}
%$\zkS$ simulates regularly until it needs to simulate the message sent by the prover in stage \ref{prover_response} of the protocol.
%Then, it takes $\zkmV$'s circuit and the FHE encryption of the target it sent earlier, $\qheE_{\qhepk}(t)$, and homomorphically evaluates $\zkmV$'s response, for an SFE encryption of $t$.
%
%If $\zkmV$ responds with a non-abort (and thus a valid response, beause the verifier is explainable and thus either aborts or gives a legal answer), we can extract by using the CC program (to be precise, we succeed in extraction with overwhelming probability over the choice of $r_\zkP$, due to the almost-perfect correctness of the CC obfuscator and the quantum FHE).
%
%If $\zkmV$ responds with an abort (which we detect by observing the output of $\obfC(\mathbf{\hat{c}'})$) then we are stuck.
%We are stuck because we had to encrypt $\zkmV$'s inner quantum state in order to homomorphically evaluate $\zkmV$'s response, and now due to the abort, we have the state encrypted and cannot output it as a simulation output - we need to output a sample from the distribution of transcripts where $\zkmV$ aborts in part \ref{verifier_response}.
%A subroutine of the simulator that is responsible for sampling such a transcript is $\zkSA$ - for the sake of understanding the main ideas in the protocol and simulator, the inner workings of this subroutine are less relevant and it can be thought of as a black box that just samples an abort transcript.
%Finally, we note that due to the fact that our access to the inner quantum state of $\zkmV$ is lost when there's an abort, our proof does not prove ZK against adversaries with quantum advice.
%
%Now, as a further explanation for $\zkSA$, a technical problem (which is not new in zero-knowledge simulations) that arises when constructing $\zkSA$, is how to keep its expected running time polynomial (a naive approch of just trying to sample an abort transcript will not necessarily be expected polynomial time, when the probability to abort in the simulated setting is negligible).
%We resolve this issue with a technique from \cite{goldreich1996construct}, with slight modifications.
%
%\medskip
%We now turn to formally proving that the simulator runs in expected polynomial time and the transcripts that it generates are computationally indistinguishable (by quantum adversaries) from the transcripts generated by the malicious verifier's real interaction with $\zkP$.
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%\begin{claim}\label{claim:sim_time}
%	Let $\zkmV = \{ \zkmV_\secp \}_{\secp \in \Nat}$, then the simulation $\zkS(\ins, \zkmV)$ runs in expected polynomial time.
%\end{claim}
%\begin{proof}
%	Denote the following probabilities:
%	\begin{itemize}
%		\item 
%		$a(x):$ the probability that $\zkmV$ aborts in part \ref{verifier_response} of the {\bf simulated} protocol (that is, in part \ref{prover_response}, the prover sent an SFE encryption $\sfeEnc_{\sfedk}(t)$ of the target).
%		\item 
%		$b(x):$ (will be useful in later claims) the probability that $\zkmV$ aborts in part \ref{verifier_response} of the {\bf original} protocol (that is, in part \ref{prover_response}, the prover sent $\sfeEnc_{\sfedk}(0^\secp)$).
%	\end{itemize}
%	Denote by $T(\ins, \zkmV)$ the running time of the simulator on input $\ins \in \lang\cap\{ 0, 1 \}^\secp$ and the verifier $\zkmV_{\secp}$, and by $T'(\ins, \zkmV)$ the running time of the subroutine $\zkSA$, thus,
%	\begin{gather*}
%	\bb{E}\left[ T(x, \zkmV) \right] = 
%	(1 - a(x))\cdot
%	\poly(\secp) + a(x)\cdot \bb{E}[T'(x, \zkmV)] \enspace ,
%	\end{gather*}
%	for some polynomial $\poly(\cdot)$ that denotes the running time of the simulator when it does not get aborts from $\zkmV$ (this polynomial depends on the circuit size of $\zkmV$, which is also a polynomial).
%	
%	Recall that the first step of $\zkSA$ is to get $\secp^2$ aborts in the simulated setting (or score $2^\secp$ iterations), thus the expected running time of this step is $\frac{\secp^2}{a(x)}$ (note that if our control path has made it to $\zkSA$, then $a(x) > 0$).
%	
%	For the second part of the abort simulation, observe that the expected running time of the second part of $\zkSA$ is bounded by
%	$$
%	\Pr\left[ a'(x) \in \left[\frac{1}{2}\cdot a(x), \, \frac{3}{2}\cdot a(x)\right] \right]\cdot \frac{2\secp}{a(\ins)}\cdot\poly(\secp) + 
%	\Pr\left[ a'(x) \notin \left[\frac{1}{2}\cdot a(x), \, \frac{3}{2}\cdot a(x)\right] \right]\cdot 2^{O(\secp)} \enspace ,
%	$$
%	thus it will be enough to show that the probability $\Pr\left[ a'(x) \notin \left[\frac{1}{2}\cdot a(x), \, \frac{3}{2}\cdot a(x)\right] \right]$ is sufficiently small.
%	We have,
%	\begin{gather*}
%	\Pr\left[ a'(x) \notin \left[\frac{1}{2}\cdot a(x), \, \frac{3}{2}\cdot a(x)\right] \right] =
%	\Pr\left[ a'(x) < \frac{1}{2}\cdot a(x) \right] +
%	\Pr\left[ a'(x) > \frac{3}{2}\cdot a(x) \right] \enspace ,
%	\end{gather*} 
%	and we use Chernoff bounds:
%	$$
%	\Pr\left[ a'(x) < \frac{1}{2}\cdot a(x) \right] \underset{(a'(\ins) = \frac{\secp^2}{N})}{\leq}
%	\Pr\left[ \frac{2\secp^2}{a(x)} < N \right] \underset{(*)}{\leq} 
%	\Pr\left[ X \leq \secp^2 \right] \leq e^{-\frac{\secp^2}{4}} \enspace ,
%	$$
%	where $(*)$ follows from using the Chernoff tail bound $\Pr\left[ X \leq (1 - \delta)\mu \right] \leq e^{-\mu\cdot\delta^2\cdot\frac{1}{2}}$, with $X$ being the number of aborts in the experiment of running the simulated protocol $\frac{2\secp^2}{a(x)}$ times, the expectation of $X$ is $2\secp^2$, and $\delta$ is $\frac{1}{2}$.
%	
%	By similar reasoning it can be easily verified that,
%	$$
%	\Pr\left[ a'(x) > \frac{3}{2}\cdot a(x) \right] \leq 
%	\Pr\left[ N < \frac{\frac{2}{3}\cdot\secp^2}{a(x)} \right]\leq
%	\Pr\left[ X \geq (1 + \frac{1}{2})\frac{2}{3}\cdot\secp^2 \right] \leq 
%	e^{-\frac{\secp^2}{15}} \enspace ,
%	$$
%	using the Chernoff tail bound $\Pr\left[ X \geq (1 + \delta)\mu \right]\leq e^{-\frac{\delta^2}{2 + \delta}\mu}$.
%\end{proof}
%
%
%
%
%
%\begin{claim}\label{fail_probability}
%	Let $\zkmV = \{ \zkmV_\secp \}_{\secp \in \Nat}$ be an explainable quantum verifier, then there's a negligible function $\mu$ s.t. for every $\secp \in \Nat, \ins \in \lang\cap\{ 0, 1 \}^\secp$: 
%	$$
%	\Pr\left[ \zkS(\ins,\zkmV_\secp) = \zkFail \right] \leq \mu(\secp) \enspace.
%	$$
%\end{claim}
%\begin{proof}
%	We have,
%	$$
%	\Pr\left[ \zkS(\ins,\zkmV_\secp) = \zkFail \right] =
%	$$
%	\begin{equation}\label{eq_1}
%	a(x)\cdot\left( \Pr\left[ \text{$\zkSA$ Failed in its first part} \right] + \Pr\left[ \text{$\zkSA$ Failed in its second part} \right] \right) \enspace ,
%	\end{equation}
%	and we start with showing that the first probability is exponentially small.
%	\begin{equation}\label{eq_2}
%	\Pr\left[ \text{$\zkSA$ Failed in its first part} \right] = 
%	\sum_{i = 0}^{\secp^2 - 1}\Pr\left[ \text{There were exactly $2^\secp - i$ fails out of $2^\secp$ tries} \right]\enspace .
%	\end{equation}
%	Now, consider two cases.
%	\begin{itemize}
%		\item 
%		$a(x) \leq 1/2:$ thus the sum from \ref{eq_2} is bounded by 
%		$$
%		\secp^2\cdot\Pr\left[ \text{There were $2^\secp$ fails} \right] = 
%		\secp^2\cdot(1 - a(x))^{2^\secp} \enspace ,
%		$$
%		and by adding the factor $a(x)$ (from \ref{eq_1}) we can split to two cases (e.g. $a(x) \leq 2^{-\secp/2}$ and $a(x) > 2^{-\secp/2}$) and show that (in both cases) when the above probability is multiplied by $a(x)$, it is bounded by $2^{-\Omega(\secp/2)}$.
%		
%		\item 
%		$a(x) > 1/2:$ thus the sum from \ref{eq_2} is bounded by
%		$$
%		\secp^2 \cdot \Pr\left[ \text{There were exactly $2^\secp - \secp^2$ fails} \right] = 
%		\secp^2 \cdot {2^\secp \choose 2^\secp - \secp^2}\cdot(1 - a(x))^{2^\secp - \secp^2}a(x)^{\secp^2} \leq
%		$$
%		$$
%		\secp^2 \cdot 2^{\secp^3}\cdot(1 - a(x))^{2^\secp - \secp^2} <
%		\secp^2 \cdot 2^{\secp^3}\cdot2^{-2^\secp + \secp^2} \leq 2^{-\Omega(2^\secp)} \enspace .
%		$$
%	\end{itemize}
%	
%	\noindent It is left to show that the probability to fail in the second step is negligible, and we calculate.
%	$$
%	\Pr\left[ \text{$\zkSA$ Failed in its second part} \right] \leq 
%	\Pr\left[ \text{There were $\frac{\secp}{a'(\ins)}$ failed trials} \right] \leq
%	$$
%	$$
%	\Pr\left[ \text{There were $\frac{\secp}{a'(\ins)}$ failed trials} \pST a'(x) \in \left[\frac{1}{2}\cdot a(x), \, \frac{3}{2}\cdot a(x) \right] \right] + 
%	\Pr\left[ a'(x) \notin \left[\frac{1}{2}\cdot a(x), \, \frac{3}{2}\cdot a(x)\right] \right] \enspace .
%	$$
%	As a part of the proof of claim \ref{claim:sim_time}, we saw that $\Pr\left[ a'(x) \notin \left[\frac{1}{2}\cdot a(x), \, \frac{3}{2}\cdot a(x)\right] \right] \leq e^{-\Omega(\secp^2)}$, so we bound the first probability.
%	$$
%	\Pr\left[ \text{There were $\frac{\secp}{a'(\ins)}$ failed trials} \pST a'(x) \in \left[\frac{1}{2}\cdot a(x), \, \frac{3}{2}\cdot a(x) \right] \right] \leq
%	$$
%	$$
%	\Pr\left[ \text{There were $\frac{2\secp}{3a(\ins)}$ failed trials} \right] =
%	(1 - b(x))^{\frac{2\secp}{3a(\ins)}} \leq
%	e^{-\frac{b(x)}{a(x)}\cdot \frac{2}{3}\cdot \secp} \enspace.
%	$$
%	
%	Assume towards contradiction that there is some noticeable probability $\varepsilon(\secp) = \secp^{-O(1)}$ s.t. for infinitely many inputs $\{ x_\secp \}_{\secp}, x_\secp \in \lang \cap\{ 0, 1 \}^\secp$, we have,
%	$$
%	\varepsilon(\secp) \leq
%	a(x)\cdot \Pr\left[ \text{There were $\frac{\secp}{a'(\ins)}$ failed trials} \pST a'(x) \in \left[\frac{1}{2}\cdot a(x), \, \frac{3}{2}\cdot a(x) \right] \right] \leq
%	a(x)\cdot e^{-\frac{b(x)}{a(x)}\cdot \frac{2}{3}\cdot \secp}
%	\enspace .
%	$$
%	Now, note that by the input privacy property of the SFE encryption, the gap $\abs{a(x) - b(x)}$ is bounded by a negligible function (if it wasn't, then by an averaging argument there is $t'\in \{ 0, 1 \}^\secp$ s.t. it is easy to distinguish between SFE encryptions of $0^\secp$ and SFE encryptions of $t'$).
%	The fact that we have both,
%	\begin{itemize}
%		\item $a(x)$ is bigger than some noticeable function.
%		\item $\abs{a(x) - b(x)}$ is bounded by a negligible function.
%	\end{itemize}
%	implies that (for large values of $\secp$) we have $\frac{b(x)}{a(x)} \in [\frac{1}{2}, 2]$, in contradiction to the inequality $\varepsilon(\secp) \leq e^{-\frac{b(x)}{a(x)}\cdot \frac{2}{3}\cdot \secp}$.
%	%\omri{from some place $\lambda$, a(x) and b(x) has to be negligibly close to each other and a(x) is also big --> b(x)/a(x) is close to constant --> the exponentiation is negligibly small --> contradiction.}
%\end{proof}
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%\medskip
%We conclude with showing that the simulation is successful.
%\begin{lemma}
%	Let $\zkmV = \{ \zkmV_\secp \}_{\secp \in \Nat}$ be an explainable quantum verifier, then,
%	$$
%	\{ \view_{\zkmV_\secp}\prot{\zkP(w)}{\zkmV_\secp}(\ins)\}_{\substack{\secp\in\Nat,\\ \ins\in\lang\cap\zo^\secp,\\ w \in \mathcal{R}_{\lang}(x)}}
%	\approx_{c}
%	\{\zkS(\ins,\zkmV_\secp)\}_{\substack{\secp\in\Nat,\\ \ins\in\lang\cap\zo^\secp,\\ w \in \mathcal{R}_{\lang}(x)}}\enspace.
%	$$
%\end{lemma}
%\begin{proof}
%	Denote by $\zkS'$ a process which is identical to $\zkS$ but when it gets an abort in \ref{check}, instead of invoking $\zkSA$, it just samples an abort transcript (from the original abort distribution, where the prover sends $\sfeEnc(0^\secp)$ in part \ref{prover_response} of the protocol).
%	By claim \ref{fail_probability}, the output distribution of this process is computationally (and in fact, even statistically) indistinguishable from the output distribution of $\zkS$.
%	All that is left to show then, is that the output distribution of $\zkS'$ is computationally indistinguishable from $\view_{\zkmV}\prot{\zkP}{\zkmV}$.
%	
%	Denote by $X_0$ the distribution of non-aborting (that is, non-aborting in step \ref{verifier_response} of the protocol) transcripts from the original interaction between $\zkmV$ and $\zkP$, and by $Y_0$ the distribution of non-aborting transcripts from the simulation.
%	Also, denote by $X_1$ the distribution of aborting transcripts from the original interaction between $\zkmV$ and $\zkP$, and by $Y_1$ the distribution of aborting transcripts from the output distribution of $\zkS'$, observe that $X_1$ and $Y_1$ are exactly the same distribution.
%	
%	We claim that $X_0$ and $Y_0$ are computationally indistinguishable (when considering their asymptotic sequences), due to the input privacy property of the SFE encryption, the special zero-knowledge property of the sigma protocol (specifically, the fact that what $\SigS(\beta)$ simulates is computationally indistinguishable from $\SigP(\beta)$'s messages), and the fact that the verifier is explainable and actually follows the coin tossing protocol and outputs legal responses (as long as it doesn't abort).
%	
%	Observe that the output distribution of $\view_{\zkmV}\prot{\zkP(w)}{\zkmV}(\ins)$ is to sample a transcript from $X_0$ with probability $1 - b(x)$, and from $X_1$ with probaility $b(x)$.
%	Also, observe that the output distribution of $\zkS'(\ins, \zkmV)$ is to sample a transcript from $Y_0$ with probability $1 - a(x)$, and from $Y_1$ with probability $a(x)$.
%	Due to the fact that $a(x)$ and $b(x)$ are negligibly close, and the pairs $(X_0, Y_0)$ and $(X_1, Y_1)$ are both computationally indistinguishable, we deduce that the output distributions of $\view_{\zkmV}\prot{\zkP(w)}{\zkmV}(\ins)$ and $\zkS'(\ins, \zkmV)$ are computationally indistinguishable (by a standard hybrid argument, distinguishing between the two output distributions will imply that either we can distinguish between $X_0$ and $Y_0$, or distinguish between $X_1$ and $Y_1$, or that the gap $\abs{a(x) - b(x)}$ is not negligible).
%	
%	\iffalse
%	uses the subroutine $\zkSA'$ instead of $\zkSA$.
%	$\zkSA'$ operates as follows: 
%	\begin{itemize}
%		\item 
%		Iterate until there is an abort (or you ran for $2^\secp$ steps, in this case output $\zkFail$):
%		simulate the prover honestly until and including part \ref{prover_response} of the protocol, and get $\zkmV$'s response on the SFE encryption of $0^\secp$.
%		If $\zkmV$ responded with $\bot$ (and there wasn't an abort in an earlier stage in this iteration) count it as an abort.
%	\end{itemize}
%	
%	%We note (without proof, for further details we refer the reader to \cite{goldreich1996construct}, Section 2, "A technical problem resolved") that $\zkS'$ does not necessarily runs in expected polynomial time, but we claim that its output distribution is computationally close to both the simulation output of $\zkS$ and $\view_{\zkmV}\prot{\zkP(w)}{\zkmV}(\ins)$.
%	\fi
%	
%\end{proof}

